On depth prediction for autonomous driving using self-supervised learning

Perception of the environment is a critical component for enabling autonomous driving. It provides the vehicle with the ability to comprehend its surroundings and make informed decisions. Depth prediction plays a pivotal role in this process, as it helps the understanding of the geometry and motion of the environment. This thesis focuses on the challenge of depth prediction using monocular self-supervised learning techniques. The problem is approached from a broader perspective first, exploring conditional generative adversarial networks (cGANs) as a potential technique to achieve better generalization was performed. In doing so, a fundamental contribution to the conditional GANs, the acontrario cGAN was proposed. The second contribution entails a single image-to-depth self-supervised method, proposing a solution for the rigid-scene assumption using a novel transformer-based method that outputs a pose for each dynamic object. The third significant aspect involves the introduction of a video-to-depth map forecasting approach. This method serves as an extension of self-supervised techniques to predict future depths. This involves the creation of a novel transformer model capable of predicting the future depth of a given scene. Moreover, the various limitations of the aforementioned methods were addressed and a video-to-video depth maps model was proposed. This model leverages the spatio-temporal consistency of the input and output sequence to predict a more accurate depth sequence output. These methods have significant applications in autonomous driving (AD) and advanced driver assistance systems (ADAS).

==> acontrario/main.tex <==
This chapter proposes two important contributions for conditional Generative Adversarial Networks (cGANs) to improve the wide variety of applications that exploit this architecture. The first main contribution is an analysis of cGANs to show that they are not explicitly conditional. In particular, it will be shown that the discriminator and subsequently the cGAN does not automatically learn the conditionality between inputs. The second contribution is a new method, called \textbf{\ac~cGAN}, that explicitly models conditionality for both parts of the adversarial architecture via a novel \ac loss that involves training the discriminator to learn unconditional (adverse) examples. This leads to a novel type of data augmentation approach for GANs (\ac learning) which allows restricting the search space of the generator to conditional outputs using adverse examples. Extensive experimentation is carried out to evaluate the conditionality of the discriminator by proposing a probability distribution analysis. Comparisons with the cGAN architecture for different applications show significant improvements in performance 
 on well known datasets including, semantic image synthesis, image segmentation, monocular depth prediction and "single label"-to-image using different metrics including Fréchet Inception Distance (FID), mean Intersection over Union (mIoU), Root Mean Square Error log (RMSE $\log$) and Number of statistically-Different Bins (NDB).

\input{acontrario/section1}
\input{acontrario/section2}
%\input{acontrario/appendix}


==> acontrario/section1.tex <==
\section{Introduction}
Since the seminal work in 2014, Generative Adversarial Networks (GANs)~\cite{goodfellow2014generative} have introduced an alternative framework for training generative models that has led to a multitude of high impact publications over a very large number of applications. Conditional GANs, introduced shortly after~\cite{mirza2014conditional}, have extended GANs to incorporate conditional information as input and have demonstrated resounding success for many computer vision tasks such as image synthesis~\cite{Isola2017ImagetoImageTW,Park2019SemanticIS,Wang2018HighResolutionIS,chen2017photographic,Sushko2020YouON,Tang2020LocalCA,Liu2019LearningTP}, video synthesis \cite{Wang2018VideotoVideoS,Chan2019EverybodyDN,Liu2019NeuralRA}, image correction\cite{Kupyn2018DeblurGANBM,Zhang2020ImageDU,Qu2019EnhancedPD}, text-to-image\cite{Reed2016GenerativeAT,zhang2018stackgan++,Xu2018AttnGANFT,Li2019ObjectDrivenTS}. In all these works, the underlying GAN model as proposed in~\cite{goodfellow2014generative} and~\cite{mirza2014conditional} have formed the basis for more advanced architectures and their properties have been analysed in detail and established in terms of convergence\cite{Kodali2018OnCA,Nie2018JRGANJR}, mode collapse\cite{Srivastava2017VEEGANRM}, Nash equilibrium\cite{Unterthiner2018CoulombGP,Farnia2020GANsMH}, vanishing gradients\cite{Arjovsky2017TowardsPM}, etc.


The conditionality of cGANs is at the crux of their theoretical contribution and its impact therefore merits in-depth analysis. 
From the existing literature it is not clear, however, if this now widely used architecture explicitly models or even learns conditionality. Empirically, the impressive results obtained with cGANs show that the generator automatically seeks to incorporate conditional variables into its generated output. Fundamentally the generator is, however, free to generate whichever output as long as it satisfies the discriminator. Therefore, the conditionality of cGAN also depends on the conditionality of the discriminator. This begs the question as to whether or not the baseline architecture of cGANs explicitly models conditionality and if not, how can the core adversarial architecture be redefined to explicitly model conditionality? This is therefore the object of this chapter.

Problems with cGANs conditionality have been observed independently for different tasks in the literature. Label-to-image tasks observe that using only adversarial supervision yields bad quality results~\cite{Sushko2020YouON,Park2019SemanticIS, Wang2018HighResolutionIS,Liu2019LearningTP}. "Single Label"-to-image tasks~\cite{Brock2019LargeSG} observes class leakage. It is also well known that cGANs are prone to mode collapse~\cite{richardson2018gans}. In this chapter it is suggested that all these problems are related to the lack of a conditional discriminator.

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{acontrario/images/pipeline.pdf}
    \caption{\small	 The classic cGAN and the proposed \ac cGAN discriminators are tested with 500 validation images of the Cityscapes dataset on both conditional and unconditional label-to-image input set.  Unconditional inputs (Real \ac and Generated \ac) set are obtained by randomly shuffling the original conditional sets of data. The classic cGAN discriminator fails to classify unconditional input set as false as seen by the histogram distributions on the right (real \ac in red is classified as true). The proposed method trains the discriminator with a general \ac loss to classify unconditional input set as fake (note that no extra training samples are required). The he proposed \ac cGAN correctly classifies all four modalities (blue, green, red, yellow) correctly.}
    \label{fig:pipeline}
\end{figure*}
Consider a simple test of conditionality on a learnt discriminator for the task of label-to-image translation, shown in Figure~\ref{fig:pipeline}. The conditional label input is purposely swapped with a non-corresponding input drawn randomly from the input set (\eg labels). From this test it is revealed that the discriminator does not succeed to detect the entire set of \ac examples (defined in Section~\ref{sec:consistency}) as false input pairs. This suggests that the generator is not constrained by the discriminator to produce conditional output but rather to produce any output from the target domain (images in this case). Furthermore, in practice, the large majority of methods that exploit cGANs for label-to-image translation, if not all, add additional loss terms to the generator to improve conditionality. These loss terms are, however, not adversarial in their construction. For example, high resolution image synthesis approaches such as~\cite{Wang2018HighResolutionIS} suffer from poor image quality when trained with only adversarial supervision~\cite{Sushko2020YouON}. Considering the well known pix-to-pix architecture~\cite{Isola2017ImagetoImageTW}, a L1 loss was introduced to improve performance. This additional term seeks to enforce conditionality on the generator but does not act explicitly on the discriminator. Subsequently, one could question if the conditionality obtained by such methods is obtained via this loss term which is not part of the adversarial network architecture. Moreover, adding an extra loss term to the generator has now become the defacto method for improving cGANs results. For example perceptual loss~\cite{Johnson2016PerceptualLF} and feature-matching~\cite{Salimans2016ImprovedTF} have been proposed and reused by many others\cite{Wang2018HighResolutionIS,chen2017photographic,Park2019SemanticIS,Ntavelis2020SESAMESE}. As demonstrated in the experiments different tasks such as image-to-depth or image-to-label also exhibit these drawbacks.

In this chapter we will be arguing that simply providing condition variables as input is insufficient for modelling conditionality and that it is necessary to explicitly enforce dependence between variables in the discriminator. It will be demonstrated that the vanilla cGAN approach is not explicitly conditional via probabilistic testing of the discriminator's capacity to model conditionality.
With this insight, a new method for explicitly modelling conditionality in the discriminator and subsequently the generator will be proposed. This new method not only offers a solution for conditionality but also provides the basis for a general data augmentation method by learning from the contrary (\ac data augmentation).

\section{Related work}


\paragraph*{Conditional GANs}
Several methods have been proposed to incorporate conditional information into the discriminator. \cite{mirza2014conditional} proposed an early fusion approach by concatenating the condition vector to the input of the discriminator.  \cite{Miyato2018cGANsWP,Kang2020ContraGANCL,Ntavelis2020SESAMESE,Liu2019LearningTP,kavalerov2021multi} proposed a late fusion by encoding the conditional information and introducing it into the final layers of the discriminator. \cite{Sushko2020YouON} replaces the discriminator with a pixel-wise semantic segmentation network. Most of these methods are task specific and not general~\cite{kavalerov2021multi,Sushko2020YouON,Kang2020ContraGANCL}. The method proposed in this chapter is a task agnostic solution for incorporating any conditional variables and it will be shown to perform on several different datasets.

One concern raised in the literature is that improving either player is at the detriment to learning and can lead to mode collapse or vanishing gradient~\cite{Arjovsky2017TowardsPM, dai2017good}. In the present chapter, whilst the aim is to define a conditional discriminator, it is argued that not only this does not affect the Nash equilibrium but also helps to avoid mode collapse and vanishing gradient. A simple example is that the proposed discriminator imposes conditionality and therefore the different condition inputs cannot be collapsed into a single mode.

\paragraph*{Data augmentation for GANs}
Data augmentation is a highly useful strategy to improve generalization for machine learning that involves increasing the diversity of training data without collecting new samples. Augmentation strategies have involved performing a variety operations on input training data including random cropping, horizontal flipping, various hand-crafted operations~\cite{hendrycks2019augmix,ghiasi2020simple} or even learning augmentation strategies from data~\cite{zhang2019adversarial,cubuk2019autoaugment}. Performing data augmentation on GANs is less straightforward and has been limited to a handful of operations such as flipping, cropping and jittering~\cite{Isola2017ImagetoImageTW}.  \cite{Zhao2020ImprovedCR,Zhang2020ConsistencyRF} propose a method to enforce the discriminator to remain unchanged by arbitrary augmentation. \cite{zhao2020image,zhao2020differentiable,Karras2020TrainingGA,9319516} study the artifacts produced by augmentation and propose to perform augmentation on both real and generated images for both generator and discriminator training. Further, \cite{Karras2020TrainingGA} proposes a method called stochastic discriminator augmentation that adjusts the augmentation strength adaptively. Alternatively to all these approaches, the \ac learning proposed in this chapter performs data augmentation by providing false counter examples rather than augmenting the real data-set with transformations. The proposed data augmentation approach is therefore specific to adversarial architectures, however, it will be shown that by discriminating against undesirable distributions, the generator is better constrained towards the target distribution. In the specific case of conditionality, by providing \ac examples to the discriminator as fakes, the discriminator constrains the generator to only learn conditional generations and the generator is therefore better constrained. It should be noted that in parallel to this work, the idea of augmenting the discriminator with fake examples was recently proposed in~\cite{sinha2020negative}, however, this method did not consider discriminator conditionality and only investigated data augmentation through creating fake data.  

\paragraph*{Evaluation criteria for GANs}
\label{sec:related_work_eval}
Defining an evaluation criteria to assess and compare GAN architectures has been a major problem in advancing the field. The difficulty and advantage of GAN architectures lies in that the learnt discriminator replaces the classic objective function. 
Classic approaches for evaluating GANs often use the FID~\cite{Heusel2017GANsTB} or Inception scores~\cite{Salimans2016ImprovedTF} to evaluate high-level generation quality and diversity. For example, the inception score only allows to evaluate a perceptual image quality and does not account for consistency between generated output and label. By construction it is therefore domain specific and does not evaluate conditionality in the output. More recent approaches investigate more general metrics~\cite{arora2017generalization,huang2017parametric,im2018quantitatively,gulrajani2020towards,zhang2018unreasonable}. Nevertheless, none of these approaches specifically allow to evaluate the conditionality of conditional GANs. Such an evaluation metric should take both the condition variables and generated variables into account.
Therefore, for the sake of evaluation, experiments were done on tasks that could provide a strong conditional metric to evaluate conditionality. The mIoU was used specifically for evaluating semantically conditional examples and $\log$ RMSE was considered for geometric depth conditionality.

\section{Method}
\label{sec:method}
The classical conditional GAN and the acontrario proposition are detailed in~\refsec{consistency} and~\refsec{ccgan}

\subsection{Evaluating conditionality} 
\label{sec:conditioneval}
The objective of this section is to propose methods to test the conditionality of cGAN networks. As mentioned in Section~\ref{sec:related_work_eval}, state-of-the-art approaches have focused on evaluating cGAN architectures with metrics applied to the generator output. Since the generator and discriminator are coupled, these metrics essentially evaluate the full GAN architecture.

A proposal is made to test the conditionality by visualizing the probability distribution at the output of the discriminator. Due to the fact that adversarial training involves a zero-sum game between a generator and a discriminator, both the generator and discriminator should seek to reach an equilibrium (Eq~\ref{eq:cost}) at the end of training. One issue for GANs is that when the discriminator dominates there is a vanishing gradient problem~\cite{Arjovsky2017TowardsPM}. It is therefore more difficult (but not impossible) to isolate the discriminator during training to evaluate its capacity to detect unconditional examples as false. For this reason, an optimal discriminator can be used to give insight for evaluation purposes as in~\cite{Arjovsky2017TowardsPM,Farnia2020GANsMH}. An optimal discriminator is essentially a binary classifier which classifies between true and fake (see Eq~\eqref{eq:classic_loss}).

In order to test the optimal discriminator, consider that the generator has been fixed after a certain number of iterations (the generator is initially random) and the discriminator has been allowed to converge to an optimal solution based on the following objective function:
 \begin{align}
    \max_{D\in \mathbb{D}} V(G_{fixed},D) 
    \label{eq:optimaldiscrim}
\end{align}


The evaluation subsequently involves analysing the distributions produced by the optimal discriminator (Eq~\eqref{eq:optimaldiscrim}) given test distributions containing unconditional or \ac sets of data-pairings. The capacity of the discriminator to correctly classify unconditional data as false is then analysed statistically. Section~\ref{sec:consistency} provides a formal definition of these unconditional data pairings. Probability distributions are visualised and evaluated by histogram analysis on the discriminator features in the last convolution layer. 


==> acontrario/section2.tex <==
\section{Experimental section}
\label{sec:experiments}
Several experiments will be presented that evaluate the conditionality of cGANs including: Real image generation from semantic masks on Cityscapes dataset~\cite{cordts2016cityscapes};"Single label"-to-image on CIFAR-10~\cite{cifar}; Monocular depth estimation on~\cite{Silberman:ECCV12}; Semantic segmentation using pix2pix on Cityscapes dataset. 
For label-to-image generation, pix2pix\cite{Isola2017ImagetoImageTW},  pix2pixHD\cite{Wang2018HighResolutionIS}, SPADE\cite{Park2019SemanticIS} and CC-FPSE\cite{Liu2019LearningTP} were used to test the conditionality and to highlight the contribution of the \ac cGAN wrt state-of-the-art approaches. "Single label"-to-image is also considered as most new techniques that improves cGANs are designed tested using this task. To demonstrate the generality of the proposed approach depth estimation and image-to-label segmentation tasks are also performed. These structured prediction problems offer strong metrics for evaluating cGANs and various public datasets are available for training. While the scope of conditional evaluation has been limited to tasks that could provide a metric to evaluate both the conditionality and the quality of the generation, the proposed approach is general and not specific to these particular tasks. During training, the network's architecture, the additional losses, the hyper-parameters
and data augmentation schemes are kept as in the original papers ~\cite{Isola2017ImagetoImageTW, Park2019SemanticIS, Wang2018HighResolutionIS, Liu2019LearningTP}. The new additional \ac term is the only difference between the compared methods. 

\subsection{Evaluating conditionality}
\label{sec:eval}
\begin{figure*}
\centering    
\includegraphics[width=0.245\textwidth]{acontrario/images/baseline_D.pdf}
\includegraphics[width=0.245\textwidth]{acontrario/images/baseline_200.pdf}
\includegraphics[width=0.245\textwidth]{acontrario/images/explicit_D.pdf}
\includegraphics[width=0.245\textwidth]{acontrario/images/explicit_200.pdf}
\caption{\small	Label-to-image histogram results when validating 500 Cityscape images on a discriminator trained until epoch 200. Blue is Generated-conditional, Green is generated \ac, Red is real-\ac, Yellow is Real-conditional. (a) The trained baseline discriminator, (b) Optimal baseline discriminator, (c) \ac cGAN discriminator, (d) Optimal \ac cGAN discriminator. (a) and (c) are still learning indicating no vanishing gradient or mode collapse~\cite{Arjovsky2017TowardsPM}. (b) doesn't detect conditionality since \ac real is classified as true (red) (d) succeeds to classify all modes correctly.}
\label{fig:dist}  
\end{figure*}

Preliminary conditionality evaluation follows the method presented in Section~\ref{sec:conditioneval} using \ac sets to evaluate an optimal discriminator. 
In a first part experiments were carried out on the vanilla pix2pix cGAN with a discriminator PatchGAN architecture with $70\times70$ receptive field. The model was trained on the Cityscapes dataset~\cite{cordts2016cityscapes} for label-to-image translation with 2975 training images resized to $256\times256$. The pix2pix GAN model is trained with the same hyper-parameters as specified in the original paper~\cite{Isola2017ImagetoImageTW}. The evaluation histogram is calculated on the values of the last convolution layer of the discriminator ($f(x,y)$ of Eq~\eqref{eq:discriminator}) based on the $500$ validation images. Each sample from the last convolutional layer is composed of a $30\times30$ overlapping patches with one channel.The proposed approach is trained in exactly the same manner with the only difference being the new objective function. 

Various tests were carried out to investigate the output distributions of each set of data for both the baseline architecture and the proposed method. The underlying accuracy of the implementation was first validated to ensure the accuracy reported in the original paper.  A histogram analysis was then performed for different levels of training including: training for 20, 100, 200 epochs and evaluating after each. In another experiment the discriminator was allowed to continue to converge for one epoch after fixing 20, 100 and 200 epochs of cGAN training. In particular, training is performed with the objective given in Eq~\eqref{eq:optimaldiscrim} and as proposed in~\cite{Arjovsky2017TowardsPM, Farnia2020GANsMH}. These results are plotted for each data pairing: real-conditional,  generated-conditional, real-\act and generated-\act in Figure~\ref{fig:dist}. 
    Figure~\ref{fig:dist} (a) and (c) show that during training the generator is still learning with no vanishing gradient or mode collapse. In Figure~\ref{fig:dist} (b) the discriminator has been allowed to reach an optimal value by fixing the generator. The real \ac pairing is wrongly classified $99.9\%$ of the time indicating that the discriminator has not learnt conditionality. (d) Shows clearly four distinct distributions and shows the ability of the proposed approach to learn conditionality and correctly classify real \ac pairing $91.9\%$ of the time. Similar conditionality tests were performed for various alternative architectures including using a separate/shared network for $\mbf{x}$ and $\mbf{y}$ and early/late/at-each-layer fusion. In all cases conditionality was not learnt. 


% TODO citing the additional mat
These results strongly suggest that classic cGAN is unable to learn conditionality and that the spectacular results obtained by cGAN architectures are largely due to higher a level style constraints that are not specific to the input condition variable since swapping condition variables produces no effect. The proposed histogram test allows to demonstrate the ability of the discriminator to classify the various underlying classes of data and shows their statistical distribution. The approach proposed in~\cite{Arjovsky2017TowardsPM, kavalerov2021multi}
% TODO or Multi hinge cGAN loss
 looks only at accuracy, while the proposed histogram test also allows to see how well the discriminator distinguishes between the different data modalities (real/fake/\ac).



\subsection{Label-To-Image translation}
\label{sec:lb-to-im}
\begin{figure*}
\centering    
\includegraphics[width=0.30\textwidth]{acontrario/images/cityscape_normal.pdf}
\includegraphics[width=0.30\textwidth]{acontrario/images/cityscape_fixed.pdf}
\includegraphics[width=0.30\textwidth]{acontrario/images/miou2.pdf}
    \caption{\small	Comparison of the proposed approach on the Cityscape label-to-image training set. (a) The loss function for each set of data-pairing for the baseline cGAN method (\ac are for evaluation only). (b) The loss function for each set of data-pairing for the \ac cGAN method. (c) The evolution of the mIOU for both methods, performed on the validation dataset. It can be seen in (b) compared to (a) that the \ac loss converges to 0 rapidly for the proposed approach. In (c) the proposed approach is much more efficient and converges much faster and with higher accuracy.}
    \label{fig:mIoU}
\end{figure*}

Generating realistic images from semantic labels is good task to evaluate the effect of the \ac at a high level since many images can be potentially generated for each semantic class label. Figure~\ref{fig:mIoU}(c) shows a comparison of the mIoU for the baseline pix2pix model and proposed pix2pix model with the additional \ac loss. It can be observed that the \ac cGAN converges faster than the baseline. The mIoU of the model with \ac at iteration $163$k is $24.46$ whereas the baseline is $14.65$. The mIoU oscillates around that value for the \ac model indicating that the model has converged. After $595$k iterations, the mIoU for both models are very close $28.28$ and $26.41$. It is worth noting that evaluating using real images yields $29.6$. The convergence is reported for the generator where the computational cost is exactly the same. the \ac loss is specific only to the discriminator and adds a small computational cost. By restricting the search space of the generator to only conditional pairs, the generator's convergence is faster.

Table~\ref{tab:high_resolution} shows a comparison of different architectures with and without \ac augmentation. For a fair comparison all the networks are trained from scratch and the same hyper-parameter are used. The \ac loss is the only difference between the two networks. The batch size for SPADE is 32 and 16 for CC-FPSE. Through explicitly enforcing the conditionality with \ac examples, the discriminator learns to penalize unconditional generation achieving better results.  

Moreover, Figure~\ref{fig:mIoU}(a) and Figure~\ref{fig:mIoU}(b) show the comparison of the losses of the discriminator for both models on this dataset. The baseline is trained with only conditional pairs, however, the \ac data pairs are plotted to asses the ability of the discriminator to learn the conditionality automatically. The \ac losses remain high for the baseline and converge to $0$ for the proposed \ac cGAN. Figure~\ref{fig:dist} presented the histogram results for this experiment showed that the proposed approach better models conditionality. Subsequently the gradients provided to the generator are expected to be better directed.

\begin{table}
    \centering
    \resizebox{0.8\textwidth}{!}{\begin{tabular}{|c||c|c|c c|}
         \hline
         Method & Resolution & FID & mIoU & Pixel accuracy (PA) \\
         \hline
         pix2PixHD & $256\times512$  & 66.7 & 56.9 & 92.8 \\
         \ac pix2pixHD &  $256\times512$ & \textbf{60.1}& \textbf{60.1} & \textbf{93.2}\\
         \hline
         SPADE & $256\times512$ & 65.5 & 60.2 & 93.1\\
         \ac SPADE & $256\times512$ & \textbf{59.9} & \textbf{61.5} & \textbf{93.7} \\
         \hline
         CC-FPSE & $256\times512$ & \textbf{52.4} & 61.8 & 92.8\\ 
         \ac CC-FPSE & $256\times512$ & 53.5 & \textbf{63.9} & \textbf{93.5} \\
         \hline
    \end{tabular}}
        \vspace{0.2cm}
    \caption{ \small	A comparison of different architectures trained from scratch with and without \ac augmentation. The networks with \ac achieves better results with a mean improvement of $\Delta mIoU= +2.3$, $\Delta PA= +0.56 $, and $\Delta FID= -3.8$.}
    \label{tab:high_resolution}
\end{table}

\subsection{Single-label-to-image}
The generality of the proposed \ac cGAN can also be demonstrated by showing that it also improves architectures other than image-to-image. An example of a different task is conditioning the generated image on a single input class-label as in~\cite{Brock2019LargeSG,Miyato2018cGANsWP,Odena2017ConditionalIS,Karras2020TrainingGA,Kang2020ContraGANCL}. This different architecture is of interest because many new methods for improving cGANs are often tested on this task. Unfortunately, these methods are mainly evaluated on the FID~\cite{Heusel2017GANsTB} and IS~\cite{Salimans2016ImprovedTF} scores. As stated earlier, these metrics measure the quality/diversity and they favor models that memorise the training set~\cite{gulrajani2020towards}. They have not been designed to evaluate conditionality and therefore not sufficient for the purpose of this chapter. 
Despite that, these criteria are still important for evaluating the quality of GANs, however, an additional criterion is required for testing conditionality. 

Here a simple conditionality test is proposed specifically for "single label"-to-image generation tasks based on a pretrained Resnet-56~\cite{he2016deep} classifier trained on CIFAR-10~\cite{cifar}. BigGAN~\cite{Brock2019LargeSG} was selected as the baseline. Since BigGAN uses the Hinge-loss~\cite{lim2017geometric}, the \ac loss is adapted as follows:
\begin{align}
        \mathcal{L}_{D}=  -&\mathbb{E}_{\mbf{x} \sim p(\mbf{x}) , \mbf{y} \sim p(\mbf{y|x})}\big[min(0, -1 + D(\mbf{x},\mbf{y})]\big] -  \mathbb{E}_{\mbf{x}\sim p(\mbf{x})}\big[min(0,-1 - D(\mbf{x},G(\mbf{x}))]\big]  \notag  \\  
        -&\mathbb{E}_{\mbf{\tilde x} \sim p(\mbf{\tilde x}) , \mbf{y} \sim p(\mbf{y})}\big[min(0,-1-D(\mbf{\tilde x},\mbf{y}))\big] - \mathbb{E}_{\mbf{\tilde x}\sim p(\mbf{\tilde x}), \mbf{x} \sim p(  \mbf{x})}\big[min(0,-1 - D(\mbf{\tilde x},G(\mbf{x})))\big] \notag \\
        \mathcal{L}_{G}= - &\mathbb{E}_{\mbf{x}\sim p(\mbf{ x})} D(\mbf{x},G(\mbf{x}))
\label{eq:HingleLoss}
\end{align}
Both models are trained from scratch on CIFAR-10~\cite{cifar} dataset using the hyper-parameter specified in~\cite{Brock2019LargeSG}. The conditionality is tested by generating 10k images for each label(100k images in total) and calculating the accuracy. The results\footnote{The Pytorch IS and FID implementations were used for comparison}are shown in Table~\ref{tab:biggan_table}.
\begin{table}[h]   
    \centering
    \begin{tabular}{|c||c|c|c|c|}
         \hline
         Method & IS score & FID score & Acc  \\
         \hline
         BigGAN\cite{Brock2019LargeSG} & 8.26 $\pm$ 0.095   & 6.84  & 86.54 \\
         \hline
         \ac BigGAN & \textbf{8.40} $\pm$ 0.067 &   \textbf{6.28} & \textbf{92.04} \\
         \hline
    \end{tabular} 
        \vspace{0.2cm}
    \caption{\small A comparison of BigGAN~\cite{Brock2019LargeSG} with and without the \ac GAN. The network with \ac achieves significantly better results with an improvement of $\Delta Acc= +5.59$, $\Delta IS= +0.14 $, and $\Delta FID= -0.56$.
    }
    \label{tab:biggan_table}
\end{table}

The conditionality improved significantly over the baseline with $\Delta Acc=+5.59$ and the quality also improved with $\Delta FID= - 0.56\:$, $ \Delta{IS}=+0.14$. Similar to the observation made before \ac enforces the conditionality without compromising the quality. A failure mode of the lack of conditionality of the discriminator is class leakage : images from one class contain properties of another. While is it not easy to define a proper metric for such failure mode, it is shown that using the \ac loss the classification was improved and therefore the generation is better constrained and does not mix class properties. This result shows that \ac GAN also improves on a different SOTA task and confirms again that conditionality is an overlooked factor in current SOTA metrics.

 
\subsection{Image-to-label segmentation}
% TODO delete the diagram and report only the performances as a table.
Image-to-label is a simpler task compared to depth prediction and label-to-image prediction as the goal of the generator is to transfer from a high-dimensional space to a lower-dimensional space. Furthermore, the evaluation is simpler since the image mask does not have multiple solutions and it is not necessary to use an external pre-trained segmentation network for comparison as in the case of label-to-image translation. It is worth mentioning that pix2pix is trained to output 19 classes as a segmentation network and is not trained as an image-to-image network as it is often done in cGAN architectures. FCN~\cite{long2015fully} trained on~\cite{Isola2017ImagetoImageTW} obtains $21.0$ mIoU. The performances are shown in Table~\ref{tab:seg_table}. The training was unstable. However, the \ac cGAN shows superior mIoU performance with $19.23$ versus $15.97$ for the baseline model. Figure~\ref{fig:seg_qualitative} shows the qualitative results of the both models. It can be observed that the model baseline has invented labels that are not specified by the input. Training with \ac helps the discriminator to model conditionality. Thus, the generator search space is restricted to only conditional space. The generator is penalized for conditionality even if the generation is realistic.   
\begin{table}  
    \centering
    \begin{tabular}{|c||c|c|c|c|}
         \hline
         Method & Pixel accuracy (PA) & Mean Acc & FreqW Acc  & mIoU  \\
         \hline
         Baseline & 66.12 & 23.31  & 53.64  & 15.97 \\
         \hline
         \ac & \textbf{72.93} &  \textbf{26.87} & \textbf{60.40} & \textbf{19.23} \\
         \hline
    \end{tabular} 
        \vspace{0.2cm}
    \caption{\small Comparison on the Cityscapes dataset validation set. The proposed method consistently obtains more accurate results and finishes with a largely different score at the end of training with mIoU of $19.23$ versus for the baseline $15.97$.}
    \label{tab:seg_table}
\end{table}

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{acontrario/appendix/im-to-label.pdf}
    \caption{Qualitative results of Cityscape image-to-label task. It can be seen that the baseline model hallucinates objects. For instance, in the second row, the baseline hallucinates cars while the \ac cGAN segments the scene better. In the first row, the baseline wrongly classifies the pedestrian as a car. While training the model, the discriminator does not penalize the generator for these miss-classifications}
    \label{fig:seg_qualitative}
\end{figure*}



\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{acontrario/appendix/label-to-im.pdf}
    \caption{Qualitative results of Cityscapes label-to-image synthesis. In line with the quantitative results reported in Section \ref{sec:lb-to-im}, the qualitative results show better results for the \ac in comparison to the baseline. }
    \label{fig:cityscapes_qualitative}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{acontrario/appendix/comparison_SOTA.pdf}
    \caption{Qualitative comparison between different state-of-the-art methods for label-to-image trained and tested on Cityscapes\cite{cordts2016cityscapes} dataset. As observed, CC-FPSE baseline is the best baseline among classic cGAN. The \ac improves all the baseline and the best model among the 6 models is \ac CC-FPSE}
    \label{fig:state_of_art_comparison}
\end{figure}
\section{Conclusion}
 
This chapter has proposed two important contributions for conditional Generative Adversarial Networks (cGANs). The first main contribution is a probabilistic analysis of the discriminator to show that it is not explicitly conditional. The second contribution is a new method, called \textbf{\ac~cGAN}, that explicitly models conditionality for both parts of the adversarial architecture via a novel \ac loss that involves training the discriminator to learn unconditional (adverse) examples. This leads to a novel type of data augmentation approach for GANs (\ac learning) which allows to restrict the search space of the generator to conditional outputs using adverse examples. Extensive experimentation has shown significant improvements across several tasks, datasets and architectures. 



==> ch2/background.tex <==
% Introdce the common background of the thesis 
\section{Machine learning basics}
Learning is the process of acquiring new knowledge or skills through experience or study. Machine learning%, an element of artificial intelligence, 
attempts to create algorithms that can gain knowledge from and make judgments or decisions depending on data. Primarily, machine learning involves designing models that are capable of extracting knowledge or insights from data employing the learning procedure.


According to Mitchell~\cite{mitchell1997machine} “A computer program is said to learn from experience $E$ with respect to some class of tasks $T$ and performance measure $P$, if its performance at tasks in $T$, as measured by $P$, improves with experience $E$.” In the context of deep learning, the computer program is a model $\hat{\mby}=f(\mbx;\bm{\mathbf{\bm{\theta}}})$ defined by its parameters $\mathbf{\bm{\theta}}$. $\mbf{x}$ is the input variable and $\hat{\mby}$ is the output of the model. 
The experience, or dataset, is a collection of examples $\mbf{D} = {(\mbx_1,\mby_1), (\mbx_2,\mby_2), ..., (\mbx_N,\mby_N)}$ where each example is a pair of input $\mbx$ and output $\mby$. The task varies depending on the user's need, \ie classification, object detection …etc. The performance measure P assesses how the model performs on the given task.  

For deep learning, the back-propagation algorithm is commonly used to learn these parameters through optimization with gradient descent. More often, the performance metric P is not differentiable and cannot be used with the back-propagation framework. In this case, a surrogate loss function is used instead. It acts as a proxy for the performance metric. By minimizing the loss function, the performance measure is improved. For example, the cross-entropy loss is the proxy loss for classification precision, and minimizing it leads to improved classification precision. Learning can be defined more formally as: 
\begin{align}
    \label{eq:risk}
    \mbf{R}(\bm{\theta}) = \min_{\bm{\theta}} \mathbb{E}_{(\mbx,\mby) \sim p_{data}(\mbx,\mby)} L(f(\mbf{x};\bm{\theta}),\mbf{y})
\end{align}
Learning involves finding the set of parameters $\bm{\theta}$ that minimizes the expected value of the loss function L across the data generating distribution $p_{data}(\mbx,\mby)$. The quantity $\mbf{R}(\bm{\theta})$ is known as the risk. In practice, however, this quantity cannot be optimized as $p_{data}(\mbx,\mby)$ is not known. Instead, the empirical distribution represented by the training set $\mbf{D}_{train}$ is used and \refeq{risk} becomes: 
\begin{align}
\label{eq:empiricalrisk}
    \mbf{r}(\bm{\theta}) = \min_{\bm{\theta}} \sum_{D_{train}} L(f(\mbf{x};\mathbf{\bm{\theta}}),\mbf{y})
\end{align}
This quantity is known as the \textbf{empirical risk} it is also known as the \textbf{generalization error}.





\subsection{Generalization}

% Talking about supervised, self-supervised and unsupervised learning. Why learning and not classical methods
Generalization is achieved when the model is capable of learning representative and abstract features that capture complex relationships and patterns in the data. In order to assess the model for generalization,~\refeq{empiricalrisk} is also calculated for the validation dataset $\mbf{D}_{val}$ : 
\begin{align}
\label{eq:empiricalrisk_val}
    \mbf{r}(\bm{\theta}) = \min_{\bm{\theta}} \sum_{D_{val}} L(f(\mbf{x};\mathbf{\bm{\theta}}),\mbf{y})
\end{align}
A model reaches good generalization when the training error~\refeq{risk} is very low and the gap between the validation~\refeq{empiricalrisk_val} and training errors~\refeq{risk} is very low. Poor generalization can be divided into two categories:
\begin{itemize}
    \item \textbf{Over-fitting :} If the gap between the training and validation generalization error is big, this indicates that the model has memorized the training set, and it is not able to generalize for unseen data. This happens when the model is too complex and has learned patterns and relationships that are specific to the training data
    \item \textbf{Under-fitting: } This is characterized when the training error and validation error are poor, the validation error may even be lower than the training error. This happens when the model is too simple, and it is not capable of learning a meaningful and useful feature.
\end{itemize}
Generalization could be improved using several techniques including regularization, increasing the dataset size, and using ensemble methods. 

\subsection{Representation learning}
 The complexity of the data can sometimes make the learning process challenging. For example, an RGB image with a resolution of 1024 x 512 and 8-bit representation contains a total of $1024 \times 512 \times 256 \times 256 \times 256 = 8.796 \times 10^{12}$ possible images. Modeling the distribution of this high-dimensional space is intractable.

Despite the fact that images are typically represented as high-dimensional data, it has been observed that natural images actually reside on a low-dimensional manifold. In other words, the set of all natural images exists in a lower-dimensional subspace of the high-dimensional space. One of the key insights behind the manifold hypothesis is that natural images exhibit a high degree of structure and regularity, which can be captured by low-dimensional representations. 
This assumption, which is central to machine learning, enables the identification of a meaningful representation of the data. The goal of learning is to find a good representation of this manifold. Good generalization occurs when the model is able to learn a good representation that not only accurately represents the training examples \ie interpolation, but can also accurately predict the behavior of examples that were not seen during training \ie extrapolation.~\reffig{manifold} illustrates how the data can be mapped onto two different manifolds. A good representation allows us to leverage it for the chosen tasks. For example, the representation \reffig{manifoldB} is better than \reffig{manifoldA} for classification, as it is easier to define the decision boundary that separates the two domains.  

\begin{figure}[h]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{ch2/Manifold2.pdf}
  \caption{This representation is not suitable for \\classification applications}
  \label{fig:manifoldA}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{ch2/manifold1.pdf}
  \caption{This representation is better suitable for classification applications as it shows clearly the decision boundary}
  \label{fig:manifoldB}
\end{subfigure}
    \caption{An example of a possible mapping of a dataset using two features}
    \label{fig:manifold}
\end{figure}


Learning algorithms can be classified into different categories based on the type of supervision they require. Supposing $\hat{\mbf{y}}=f(\mbf{x};\bm{\theta})$ we can make the following definitions :

\begin{itemize}
    \item \textbf{Supervised learning:} In this setting the ground-truth $\mby$ is known, and it is leveraged when calculating the loss function. The model is trained on a labeled ground-truth dataset, and it makes predictions based on this input/output mapping. Some examples of supervised learning tasks include classification: Predicting which category a new example belongs to (e.g., spam or not spam); and regression: Predicting a continuous value (e.g., the depth of an object in the scene).
    
    \item \textbf{Unsupervised learning} The model does not have access to the ground-truth labels. the model is trained to discover the underlying pattern of the data.  Some examples of unsupervised learning tasks include image generation, clustering, and domain adaptation. 

    \item \textbf{Self-supervised learning} is a special class of unsupervised learning where the model is trained against a proxy task, and when improving the proxy the downstream task is also improved. An example of self-supervision is self-supervised depth prediction. the proxy task is the image reconstruction and the depth is the downstream task. Training this model for image reconstruction provides a sufficient gradient signal to supervise the depth.  

    \item \textbf{Semi-supervised} These models leverage both supervised and unsupervised techniques. When working with partially labeled datasets, it can be beneficial to incorporate both supervised and unsupervised techniques in order to make the most of the available data, especially when the labeling cost is high. 

    
\end{itemize}
Based on the applications, we could also distinguish two types of models: generative models and predictive models. For a dataset $p_{data}(\mbx,\mby)$, the generative models try to model the distribution of the data $p(\mbx)$. Predictive models on the other hand model the distribution of the output y as $p(\mby|\mbx)$ usually y have small dimensions such as a class label.

%% add a section on its applcations with citations and 



\subsection{Generative models}
% Introduce the concept of a generative model , as an example GAN and its applications 
Generative models aim to model the distribution of $p(\mbf{x})$ or a conditional distribution $p(\mbf{x}|\mbf{y})$ such as $\mbf{y}$ is the label of $\mbf{x}$. By learning the distribution of the dataset, it is possible to generate new samples $\mbf{x}_{sythetic} \sim p(\mbf{x})$. Application of these models includes image generation, text generation, text-to-images, image-to-image translation, domain adaptation. 
The most used generative models are: Variational auto-encoders (VAEs), Generative adversarial networks GANs, and Diffusion models.


\subsubsection{Variational auto-encoders}
An autonecoder is a neural network that is used to reconstruct its input. It consists of an encoder that models $p(\mbf{h}|\mbx)$ and a decoder that models $p(\mbx_{rec}|\mbf{h})$. AE can be used as a generative model by leveraging the decoder. an auto-encoder defines a generative model of the form:  
\begin{align}
    \label{eq:autoencoder}
    p_{model}(\mbf{x}) = \int p(\mbf{x}|\mbf{h})  \: p(\mbf{h}) dh
\end{align}
Where $h$ is the latent variable. If the autoencoder is trained as a generative model, it is optimized to maximize the likelihood of $p_{model}(\mbf{x})$ with respect to $p_{data}(\mbf{x})$. However, the exact inference of \refeq{autoencoder} is intractable. It is possible to approximate this quantity using the evidence lower bound defined as follows: 
\begin{align}
    p_{model}(\mbf{x}) &=   \int p(\mbf{x}|\mbf{h})   p(\mbf{h}) dh \\ 
    log [p_{model}(\mbf{x})]  &= log \big[\int p(\mbf{x}|\mbf{h})   p(\mbf{h}) \frac{ q(\mbf{h}|\mbf{x})}{ q(\mbf{h}|\mbf{x})} dh \big]   \\ 
    log [p_{model}(\mbf{x})]  &= log \big[E_{q(\mbf{h}|\mbf{x})} \big[ \frac{ p(\mbf{x}|\mbf{h})   p(\mbf{h})}{q(\mbf{h}|\mbf{x})}   \big]    
\end{align}
Using Jansen inequality : $E[log(z)] \geq log E[z]$ :  
\begin{align}
    log [p_{model}(\mbf{x})] \geq E_{q(\mbf{h}|\mbf{x})} \Big[ log \big[\frac{ p(\mbf{x}|\mbf{h})   p(\mbf{h})}{q(\mbf{h}|\mbf{x})} \big] \Big]
     =  E_{q(\mbf{h}|\mbf{x})} p(\mbf{x}|\mbf{h}) +  E_{q(\mbf{h}|\mbf{x})} \frac{ p(\mbf{h})}{q(\mbf{h}|\mbf{x})} 
\end{align}
Further simplifying with the KL-divergence : 
\begin{equation}
    \label{eq:ELBO}
    log [p_{model}(\mbf{x})] \geq E_{q(\mbf{h}|\mbf{x})} p(\mbf{x}|\mbf{h}) - D_{KL}(q(h|x) \parallel q(h)) 
\end{equation}
maximizing~\refeq{ELBO} is equivalent to maximizing the likelihood of the decoder's output and minimizing the distance of the distribution $q(\mbf{h}|\mbx)$ and $p(\mbf{h})$. q is chosen to be a Gaussian distribution. This second term makes the approximate posterior distribution $q(\mbf{h} | \mbf{x})$ and the model prior p(h) approach each other.

The VAE model is both elegant, theoretically pleasing, and simple to implement. It also achieves good results and is among the leading approaches in generative modeling. However, when used in image generation, the output of the model tends to be blurry. One possibility is that the blurring is an intrinsic effect of maximum likelihood. The denoising VAE provides the base for other models, such as Diffusion models.


\subsubsection{Generative adversarial networks (GANs)}
Generative Adversarial Networks (GANs)~\cite{goodfellow2020generative} have introduced an alternative framework for training generative models that have led to a multitude of publications with high impact over a very large number of applications. The training of these models involves two networks that compete against each other. A generator that models the distribution $p(\mbf{x})$. It tries to fool the discriminator by generating samples that are as close as possible to real samples. The discriminator models $p(real|\mbf{x})$. The discriminator tries to classify the real and synthetic samples. This is formulated as a zero-sum game between two networks G and D competing to reach a Nash equilibrium. This game is commonly formulated through a min-max optimization problem as follows : 
    \begin{align}
        \min_{G\in\mathbb{G}}\max_{D\in\mathbb{D}} V(G,D) \label{eq:cost}
    \end{align}
The function $V$ determines the payoff of the discriminator. The discriminator receives $-V(G, D)$ as its own payoff, and the generator receives $V(G,D)$ as its own payoff. In other words, this formulation could be interpreted as a learned loss function as the discriminator provide the supervision signal to update the generator. A common way to supervise the discriminator is based on the cross entropy : 

\begin{align}
 \mathcal{L}_{adv}= \min_{G} \max_{D} \: \mathbb{E}_{(\mbf{x})\sim p_{data}(\mbf{x})}log [D(\mbf{x})] +  \mathbb{E}_{\mbf{z}\sim p_(\mbf{z})}log[1 - D(G(\mbf{z}))] 
 \label{eq:gan_classic_loss}  
\end{align}
At convergence, the generator’s samples are indistinguishable from real data, and the discriminator outputs $\frac{1}{2}$ everywhere. 
 Conditional GANs~\cite{mirza2014conditional}, introduced shortly after, have extended GANs to incorporate conditional information as input and have demonstrated resounding success for many computer vision tasks such as image synthesis~\cite{Isola2017ImagetoImageTW,Park2019SemanticIS,Wang2018HighResolutionIS,chen2017photographic,Sushko2020YouON,Tang2020LocalCA,Liu2019LearningTP}, video synthesis \cite{Wang2018VideotoVideoS,Chan2019EverybodyDN,Liu2019NeuralRA}, image correction\cite{Kupyn2018DeblurGANBM,Zhang2020ImageDU,Qu2019EnhancedPD}, text-to-image\cite{Reed2016GenerativeAT,zhang2018stackgan++,Xu2018AttnGANFT,Li2019ObjectDrivenTS}. In all these works, the underlying GAN model as proposed in~\cite{goodfellow2014generative} and~\cite{mirza2014conditional} have formed the basis for more advanced architectures and their properties have been analysed in detail and established in terms of convergence\cite{Kodali2018OnCA,Nie2018JRGANJR}, mode collapse\cite{Srivastava2017VEEGANRM}, Nash equilibrium\cite{Unterthiner2018CoulombGP,Farnia2020GANsMH}, vanishing gradients\cite{Arjovsky2017TowardsPM} \\\\
\textbf{Conditional GANs}

 A GAN is considered conditional~\cite{mirza2014conditional} when the generator's output is conditioned by an extra input variable $\mathbf{y}$ such that $G(\mathbf{y})\approx=p(\mathbf{x}|\mathbf{y})$ and discriminator's output is conditioned such that $D(\mathbf{x},\mathbf{y}) \approx p(\mathbf{z}|\mathbf{x,y})$ where $\mathbf{z}$ is the probability of the input being true or generated given $(\mathbf{x},\mathbf{y})$. 
The condition variable can be any kind of information such as a segmentation mask, depth map, image, or data from other modalities. In the literature there are various methods that have been proposed for incorporating conditional information into the generator including the introduction of new modules: Conditional Batch Normalization (CBN)~\cite{Vries2017ModulatingEV}, Conditional Instance Normalization (CIN)~\cite{Dumoulin2017ALR}, Class Modulated Convolution (CMConv)~\cite{Zhou2020SearchingTC}, Adaptive Instance Normalization~(AdaIN)~\cite{Huang2017ArbitraryST}, Spatial Adaptive Normalization (SPADE)~\cite{Park2019SemanticIS}. Recently,~\cite{Tang2020LocalCA} introduced a classification-based feature learning module to learn more discriminating and class-specific features.
Additional generator losses have also been proposed including feature matching~\cite{Salimans2016ImprovedTF}, perceptual loss~\cite{Johnson2016PerceptualLF}, and cycle-consistency loss~\cite{zhu2017unpaired}. All these methods propose approaches that improve the conditionality of the generator, however, they do not act on making the discriminator conditional.  

% Discriminator improvements
Alternatively, several methods have been proposed which investigate how to incorporate conditional information into the discriminator of adversarial networks. \cite{mirza2014conditional} proposed an early fusion approach by concatenating the condition vector to the input of the discriminator.  \cite{Miyato2018cGANsWP,Kang2020ContraGANCL,Ntavelis2020SESAMESE,Liu2019LearningTP} proposed a late fusion by encoding the conditional information and introducing it into the final layers of the discriminator. \cite{Sushko2020YouON} replaces the discriminator with a pixel-wise semantic segmentation network. Several papers improve results by adding various loss terms to the discriminator~\cite{Li2017TripleGA,Odena2017ConditionalIS,Dong2019MarginGANAT,chen2019self}, however, they don't explicitly focus on testing and constraining the conditionality of the discriminator. 
% TODO multi hinge loss
Similar to\cite{Miyato2018cGANsWP}, \cite{kavalerov2021multi} proposes an auxiliary classifier to the discriminator and use of Crammer-Singer multi-hinge loss to enforce conditionality. However, this method is task specific to only generation conditioned on class labels. 





\subsection{Predictive models}
\label{sec:predictive-model}
% Very important section to establish the definitions of prediction, infrence and forecasting
Predictive models aim to model the distribution of $p(\mbf{y}|\mbf{x})$ such that $\mbf{y}$ is a low-dimensional label for the input $\mbf{x}$. Prediction, estimation, inference and forecasting, these terms are used interchangeably in the literature and depend on the context of the task. However, we provide a more formal definition to these terms. 

\begin{itemize}
    \item \textbf{Prediction}: as mentioned earlier, predictive models aim to model the distribution of $p(\mbf{y}|\mbf{x},\bm{\theta})$. For a new measurement, $\mbf{x}_{new}$, these models "predicts" a new $\mbf{y}_{new}$. Prediction could be related to time such as predicting the $y_{t+n}$ based on $x_t$ that is modeling, $p(\mbf{y_{t+n}}|\mbf{x_t};\bm{\theta})$ or not related to time such as predicting the bounding box of an object that is modeling $p(\mbf{b}|\mbf{x};\bm{\theta})$ and $\mbf{b}$ is the bounding box of an object present in the image $\mbf{x}$.
    
    \item \textbf{Inference:} This term is often used in the literature to determine the latent variables that generate the data we observed $p(\mbf{h}|\mbf{x})$. In the deep learning community, the term inference and prediction are interchangeable~\cite{murphy2022probabilistic}, Both aim to model a distribution of some variable $\mby$ given some other variable $\mbx$ \ie $p(\mbf{y}|\mbf{x};\bm{\theta})$ but they focus on different aspects of this process. Inference involves determining the distribution of latent variables based on the observed data. One common method for doing this is Bayesian inference or using approximate inference. While prediction is used to determine the actual output $\mbf{y}$ of the predictive model. %In other words, prediction involves determining the distribution of the output variable based on the input variables.

    
    \item \textbf{Forecasting: }it is a specialized formulation of prediction that is concerned with predicting the future value 
    $\mbf{y_{t+n}}$ based on the present and the past measurements $\mbf{x_{t-k:t}}$. It models the distribution $p(\mbf{y_{t+n}}|\mbf{x_{t-k:t}})$  

    
    \item \textbf{Estimation}: Kent \ea~\cite{kent2001estimation} defines the process of estimation as "using the value of a statistic derived from a sample to estimate the value of a corresponding population parameter". In the context of deep learning, it involves finding the model parameters that minimize the error between the model's predictions and the true values of the output variables.
\end{itemize}

\section{Computer vision basics}
% Short intro about computer vision
Computer vision deals with how computers can understand and interpret images and videos. It involves the development of algorithms that can analyze and understand the environment represented as a set of \textbf{image}, Understanding this environment involves recognizing the entities and their \textbf{motion} and reasoning about their interactions. this enables to perform useful tasks such as object recognition, image classification, scene understanding, object tracking, 3D reconstruction and more. In the following section, we begin to define the rigid-body transformation and the process of acquiring images and the geometry of multiple-views.


\subsection{Rigid-body transformation}
In order to describe the motion of an object, in principle, the trajectory of all points of that objects should be specified. However, as this object do not have any deformation or change in its shape, specifying the motion of one point is sufficient. This known as rigid-body transformation. This type of transformation can include rotations, translations, and combinations of both. In the context of computer vision, rigid-body transformation is often used to describe the movement of objects within an image or video, and can be used to track the motion of those objects over time. It could be defined formally as : \\ 
% defintion of SE(3)
\textbf{Rigid-body transformation: }A map $g : \mathbb{R}^3\longrightarrow\mathbb{R}^3$ is a rigid-body transformation if it preserves the norm and the cross product of  any two vectors : 
\begin{enumerate}
    \item norm : $||g(\mbf{v})|| = ||\mbf{v}|| , \mbf{v} \in \mathbb{R}$. 
    \item cross product: $g(\mbf{v}) \times g(\mbf{u}) = g(\mbf{v} \times \mbf{u}) \mbf{v},\mbf{u} \in \mathbb{R}^3$.
\end{enumerate}
Rigid-body transformation can include rotations, translations, and combinations of both. For example, A point in the world frame at instance  $p_{1}^w$ can be transformed with a rotation and translation as shown in the \reffig{rigid_body}. The equation that relates the two points can be expressed as: 
\begin{align}
    \label{eq:rigid-body}
    p_{2}^w =^{2}R_{1} p_{1}^w + ^{2}T_{1}
\end{align}
where $^{2}R_{1}$ is the rotation matrix and  $^{2}T_{1}$ is the translation matrix.
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{ch2/rigid_body.pdf}
    \caption{An example of a rigid-body transformation}
    \label{fig:rigid_body}
\end{figure}

\subsubsection{Rotation matrix representation}
The rotation matrix is $3\times3$. However, a rotation have only $3$-DOF. Therefore, this 9 parameters matrix could be expressed using only 3 parameters. There exists several minimal parametrization of the rotation matrix such as Euler angles, quaternions and axis-angle parametrization. 

\begin{itemize}
    \item \textbf{Euler angles :} a commonly used method for rotation representation, where a rotation is decomposed into three consecutive rotations around different axes, as shown in \reffig{euler}. The simplicity and ease of interpretation of Euler angles make them a popular choice in many applications. However, it is important to note that Euler angles are not unique and can produce the same rotation with different parametrization depending on the order of the rotations.
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{ch2/euler.pdf}
    \caption{An example of an Euler rotation representation $Z_1Y_2Z_3$. Consider a Cartesian coordinate.  In order to define Euler angles, three canonical rotations are applied. First rotate around the z-axis by $\phi$, then around the new y-axis by $\bm{\theta}$, and finally around the new z-axis by $\psi$.}
    \label{fig:euler}
\end{figure}

    \item \textbf{Axis-angle representation} It represents the rotations with a single angle and axis of rotation. The axis of rotation is defined as a unit vector in 3D space, and the angle represents the magnitude of rotation about this axis. \reffig{axis-angle} represents an example of axis-angle rotation convention. The rotation is parameterized by the vector $\bm{\theta}= \theta \mbf{e}$ where the vector $\mbf{e}$ gives the direction and $\theta$ is a scalar that gives the angle.

\end{itemize}

Axis-angle representation of rotation is generally considered to be better than Euler angles in several ways:
\begin{itemize}
    \item \textbf{Unique representation:} Axis-angle provides a unique representation for a rotation, while Euler angles can lead to singularities and result in multiple solutions for a single rotation.
    \item \textbf{Avoiding Gimbals lock:} Euler angles can suffer from Gimbals lock, a phenomenon where two of the rotational degrees of freedom become locked to each other, causing the rotation to become ambiguous. Axis-angle does not suffer from Gimbals lock.

\end{itemize}
    \begin{figure}
        \centering
        \includegraphics[width=0.25\textwidth]{ch2/Axis-Angle.pdf}
        \caption{An example of the axis-angle rotation convention. The rotation is parameterized by the vector $\bm{\theta}= \theta \mbf{e}$ where the vector $\mbf{e}$ gives the direction and $\theta$ is a scalar that gives the angle.}
        \label{fig:axis-angle}
    \end{figure}

\subsubsection{Homogeneous representation}
Since \refeq{rigid-body} combine an addition and multiplication, it is possible to represent that equation with a single matrix multiplication. This is achieved by introducing a homogeneous vector, which is a 4-dimensional vector that includes an additional element of 1 at the end $\mbf{p} = (x,y,z,1)$. 

The homogeneous transformation is represented as a $4\times4$ matrix, where the first $3\times3$ elements represents the rotation and the last column represents the translation. This matrix can be used to transform a $3D$ point in one coordinate system to another coordinate system by matrix multiplication. The advantage of using a homogeneous transformation is that it allows for a compact and efficient way to represent both rotation and translation, as well as combining multiple transformations into a single matrix multiplication.

\begin{align}
    \mbf{p}_1 = \mbf{T} \mbf{p}_2 = \begin{bmatrix}
    \mbf{R} & \mbf{t} \\
    \mbf{0}_{3}& 1
    \end{bmatrix}\mbf{p}_2
\label{eq:homogenous}
\end{align}
$\mbf{T}$ is the homogeneous matrix that transforms the homogeneous point $p_1$ into the point $\mbf{p}_2$ 

It is important to note that the pose of an object refers to its position and orientation in space. It is often represented by a combination of translation $(x, y, z)$ and rotation (roll, pitch, yaw) parameters, or as a $4\times4$ transformation matrix that describes the same information.
The rigid-body transformation, on the other hand, is a mathematical operation that describes how points in one coordinate system can be transformed to another coordinate system, while preserving the distances and angles between points. It is often used to describe the relationship between two different coordinate systems. Therefore, the pose of an object or a camera describes its location and orientation in a particular coordinate system, while the rigid-body transformation describes how to transform points between two different coordinate systems.

\subsection{Pinhole camera model}
A camera is a device that captures images by detecting and measuring the intensity of electromagnetic radiation, such as light. It consists of a lens and a light sensor. The lens is used to control the direction and intensity of the incoming light, while the light sensor measures the amount of light that falls on it and converts it into an electrical signal. This measurement, known as irradiance, is a measure of the power per unit area of the light incident on the sensor, and it is typically expressed in watts per square meter $(W/m^2)$. There are several types of cameras that use different approaches to capture and process images, including pinhole cameras, fish-eye cameras, and event-based cameras. Pinhole cameras are the most common and widely used type of camera, and they are found in a wide range of applications, including smartphones, webcams and even cars. These cameras are cheap and well-documented. 


An image is a representation of the visual perception of the world. This representation encodes the world in a $2D$ array of pixels. Each of these pixels stores the color intensity for that location of the image. More Formally, an image is mapping $I$ that assign to a location $(x,y)$ a positive value : 
\begin{align}
    \mbf{I}(x,y) : \mathbb{R}^2 \Longrightarrow \mathbb{R}^{3+}
\end{align}
 An RGB image stores the color intensity of red, green and blue. For a digital image, the value of the intensity $\mbf{I}(x,y)$ is discretized in 8 or 16 bit representation. The domain of $(x,y)$ is also discretized $(x,y) \in ((0,W) \in \mathcal{N}, (0,H) \in \mathcal{N})$. Where $W$ is the width and $H$ is the height of the image.

\subsubsection{Geometric model for pinhole camera image formation}
In order to accurately model and predict the behavior of a pinhole camera, it is necessary to define a mathematical model that describes the relationship between the input light and the output image. This model takes into account the properties of the lens and sensor. By understanding and applying this mathematical model, it is possible to establish a correspondence between the points in the 3D space and their project 2D image. The pinhole camera model is shown in \reffig{pinhole-model}

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{ch2/pinhole_camera.pdf}
    \caption{Fronto-prallel pinhole camera model. The point P in the world frame is projected to the image coordinates. This process is defined using the extrinsic matrix that relates the world frame and camera frame, The projection to the image frame using the focal length and The image frame transformation using the optical center.}
    \label{fig:pinhole-model}
\end{figure}

One mathematical model that can describe the image formation includes 3 transformations : 

\begin{enumerate}
    \item \textbf{Projection into camera frame:} it transforms the point from the world frame into the camera frame : if $P_c$ have the coordinates $P_w = [X_w,Y_w,Z_w]$ we could obtain the coordinates of this point relative to the camera frame given by the rigid body transformation :
    \begin{align}
        \mbf{P_c} = ^c\mbf{T}_w \mbf{P}_w =   \begin{bmatrix}
    \mbf{R} & \mbf{t} \\
    \mbf{0}_{3}& 1
    \end{bmatrix} \mbf{P}_w 
    \end{align}

     \item \textbf{Projection into the image coordinate:} Using the fronto-parallel pinhole camera model, the 3D point $P_c$ is projected to the image frame coordinates :  
    \begin{align}
        \mbf{p} &= \begin{bmatrix}
            x \\y
        \end{bmatrix} = \frac{f}{Z} \begin{bmatrix}
            X \\Y
        \end{bmatrix}  \\ 
        Z \mbf{p} &= \begin{bmatrix}
            f  & 0  & 0 &0 \\
            0  & f  & 0 &0  \\
            0  & 0  & 1 &0 
        \end{bmatrix} \begin{bmatrix}
            X \\ Y \\ Z \\ 1
        \end{bmatrix}  = \mathbf{K}_f \begin{bmatrix}
            X \\ Y \\ Z \\ 1
        \end{bmatrix} 
    \end{align}
    $f$ represents the focal length of the camera.
    \item \textbf{Coordinates transformation from normalized coordinates to pixel coordinates:} first converting from metric to pixels and converting the origin to be the top-left of the image. This transformation can be expressed as :
    \begin{align}
       Z \begin{bmatrix}
       x' \\ y ' \\ 1
       \end{bmatrix} =  \begin{bmatrix}
            s_x  & s_{\bm{\theta}}  & o_x \\
            0  & s_{y}   & o_x \\
            0  & 0  & 1 
        \end{bmatrix} \begin{bmatrix}
            x \\ y \\ 1
        \end{bmatrix} 
    \end{align}
    $s_x$ and $s_y$ converts the metric coordinates into the pixel coordinates. $s_{\bm\theta}$ is the \textit{skew} factor usually close to zero for digital cameras. $o_x$ and $o_y$ are the coordinates of the optical center.
\end{enumerate}

In summary, the pinhole camera model can be defined as follows: 

\begin{align}
    Z \begin{bmatrix}
       x' \\ y ' \\ 1 \end{bmatrix} &= \begin{bmatrix}
            f s_x  & f s_{\bm{\theta}}  & o_x \\
            0  & f s_{y}   & o_x \\
            0  & 0  & 1 
        \end{bmatrix} \begin{bmatrix}
            1  & 0  & 0 &0 \\
            0  & 1  & 0 &0  \\
            0  & 0  & 1 &0 
        \end{bmatrix} \begin{bmatrix}
    \mbf{R} & \mbf{t} \\
    \mbf{0}_{3}& 1
    \end{bmatrix} \begin{bmatrix}
            X_w \\ Y_w \\ Z_w \\ 1
        \end{bmatrix} \\
    Z \mbf{p}' &= \mbf{K} \: \bm{\Pi} \: \mbf{T} \: \mbf{P}_w
\end{align}
Where $\mbf{K}$ is the intrinsic camera matrix. $\bm{\Pi} $ is the projection matrix, and $\mbf{T}$ is the extrinsic parameters. 

\subsubsection{Epipolar geometry}
Epipolar geometry is a mathematical concept that describes the relationship between two views of the same scene. Consider two images $(\mbf{I}_1$, $\mbf{I}_2)$ of the same scene from a different view. If a point $\mbf{X}$ have coordinates $\mbf{x}_1$ and $\mbf{x}_2$ relative to the frames of each camera and $^1T_2$ is the pose of the second camera with respect to the first then: 
\begin{align}
    \label{eq:pose}
    \mbf{x}_1 = ^1T_2 \mbf{x}_2
\end{align}
\textbf{Epipolar constraint:} The epipolar constraint that relates the two images $x_1$ and $x_2$ is defined as follows: 
    $$\mbf{x}_2^T \hat{\mbf{T}}\mbf{R} \mbf{x}_1 = 0$$
The matrix $$\mbf{E} = \hat{\mbf{T}}\mbf{R} $$ is called the essential matrix. It encodes the relative pose of the two cameras. 
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{ch2/epipolar.pdf}
    \caption{Illustration of the epipolar geometry model of two cameras with optical centers $O_1$ and $O_2$. The point $X$ is projected as $x_1$ for the first camera and $x_2$ for the secod camera. The epipoles are defined at the intersection of the image planes and the plane $(O_1,O_2,X)$. The projection of the line $(O,x_1)$ on the other camera is called the epipolar line. The corresponding point $x_2$ is situated at that line. Adopted  from~\cite{romero2020validation}}
    \label{fig:epipolar}
\end{figure}
\reffig{epipolar} show the projection, the point $\mbf{X}$ in the view. The intersection of the line $(o_1, o_2)$ is called \textbf{epipoles} denoted by $e_1, e_2$. The lines $l_1$ and $l_2$ are called the \textbf{epipolar lines} which are the intersection of the plane $(O_1,O_2,X)$ with the two image plane.

The epipolar geometry is a powerful tool for establishing correspondences between stereo pairs and resolving the scale ambiguity in depth prediction with deep learning. It is possible to project a IR pattern to replace one of the images and to establish the correspondence based on the captured pattern and the ground truth pattern this is the principle of an active depth sensor. 













\section{Image segmentation}
% Talk about segmentation in general 

Intelligent systems require the ability to reason about their environment in order to make accurate decisions. However, the raw representation of image intensity (i.e., a pixel value matrix) is not adapted to this goal. A more abstract representation is required, where each pixel encodes a more abstract information rather than an intensity value. This representation is known as segmentation. Image segmentation involves dividing an image into distinct meaningful domains, transforming it into a simplified, high-level representation. This type of representation has received a lot of attention in recent years due to its wide range of applications, including autonomous driving, medical imaging, etc. There are three main types of segmentation: semantic segmentation, instance segmentation and panoptic segmentation.

\subsection{Semantic segmentation}
Semantic segmentation is a form of image segmentation that assigns class labels to each pixel within an image, where these class labels correspond to objects or regions present within the image. For instance, in a semantic segmentation of a city street, pixels associated with the road, buildings, trees, sky, and other objects would be assigned different class labels. This approach to segmentation is valuable for tasks such as scene understanding, object detection, and scene labeling. 

In recent years, there has been substantial progress in the field of semantic segmentation. Classical methods were based on hand-crafted features. These models are limited by the representation as it does not fully capture high-level and low-level relations, thus limiting their performance. With the recent advance of deep learning methods, researchers have extended such methods to semantic segmentation. (FCNs)~\cite{long2015fully}, revolutionized the field of semantic segmentation. It is an encoder-decoder architecture where the encoder is based on the VGG-16~\cite{simonyan2014very} architecture, and the decoder consists of convolution and transposed convolution layers. The subsequent SegNet~\cite{badrinarayanan2017segnet} architecture introduced novel layers for upsampling in place of transposed convolutions, while ParseNet~\cite{liu2015parsenet} modeled global context directly. The PSPNet~\cite{zhao2017pyramid} architecture focused on multi-scale features, proposing pyramid pooling to learn feature representations at different scales. DeepLabV3+~\cite{chen2018encoder} proposed the Atrous Spatial Pyramid Pooling (ASPP) module to improve the receptive field of the backbone.  

With the advent of transformers and visual transformer (ViT)~\cite{Vaswani}, several methods were proposed.~\cite{carion2020end} proposed a hybrid architecture with a CNN based backbone and a transformer encoder-decoder to perform as semantic segmentation decoder. (ViT)~\cite{dosovitskiy2020} has proposed the first end-to-end backbone transformer based model for segmentation. Swin transformers~\cite{liu2021swin} made it possible to process high resolution images efficiently. With the success of multi-modalites pre-training on video audio and text, semantic segmentation have benefitted from this advancement. ~\cite{su2022towards} combined all the pre-training paradigm, including supervised pre-training, weakly-supervised and self-supervised resulting in an state-of-art results on ADE20K benchmark~\cite{zhou2017scene}.~\cite{chen2022vision} pretrained a model on image, text and used an adapter to introduce the image-related inductive biases into the model.


 

\subsection{Instance segmentation}
Instance segmentation aims to recognizing individual instances of objects within the image. This is particularly useful for tasks like object tracking and counting, or for identifying specific instances of objects for further analysis. For instance, in an instance of segmentation of a street scene, individual cars and bicycles would be distinguished and separated from one another.

Mask R-CNN~\cite{he2017mask} is one of the most popular models for.~\reffig{maskrcnn} Shows the architecture of the mask-RCNN model. Similar to~\cite{ren2015faster}, this model consists of a backbone that extracts the features from the image. Typically, a ResNet\cite{chen2018encoder}. In the first stage, A $RPN$ network uses these features to propose $N$ possible object in the scene. For the second stage, This method proposed a~\textit{RoIAlign} module that pools the features with better alignment to the input, and incorporates an additional object segmentation branch, in parallel to the bounding box regression and classification branch of ~\cite{ren2015faster}. Further advancements have been made with proposal based networks~\cite{liu2018path,li2017fully,chen2020blendmask}, single stage network proposal free-networks~\cite{bolya2019yolact,fu2019retinamask,lee2020centermask}, and transformers based networks~\cite{chen2021simple,chen2021simple,guo2021sotr}.

\begin{figure}
    \centering
    \includegraphics[width=0.75\textwidth]{ch2/teaser.pdf}
    \caption{Overview of Mask-RCNN architecture. Similar to ~\cite{ren2015faster}, after extracting the features of an object proposal from image, the RoIAlign module is used to pool the features of tha object. 3 Parallel heads are used after, the bounding box regression head, the class head, and the mask head. Figure adopted from~\cite{he2017mask}}
    \label{fig:maskrcnn}
\end{figure}
\subsection{Panoptic segmentation}
Panoptic segmentation combines semantic segmentation with instance segmentation. This task is represented with a foreground/background classes. The fourground ‘thing’ class represents countable categories in the real world, such as people, cars. Each of these objects is assigned a unique identifier along the object mask. The background ‘stuff’ class represents categories that cannot be counted, such as road and wall. It was shown that combining these two tasks improves the performance for both tasks. 
The introduction of panoptic segmentation was first presented in the seminal work of Kirillov \ea~\cite{kirillov2019panoptic}. The authors of this work formulated the task, established evaluation parameters, and presented a basic baseline. Since then, the task has received considerable attention in the research community, resulting in numerous techniques and approaches~\cite{mohan2021efficientps,kirillov2019panoptic,chen2020banet,chen2020spatialflow,wang2020axial,chen2020panonet}.

 EfficientPS~\cite{mohan2021efficientps} is a panoptic segmentation networj that improves upon EfficientNet~\cite{tan2019efficientnet} by proposing 2-way FPN that both encodes and aggregates semantically rich multiscale features in a top-down and bottom-up way.~\reffig{panoptic-seg} shows the architecture EfficientPS. This model consists of a shared backbone, EfficientNet~\cite{tan2019efficientnet}, the complexity of this model could be controlled. The two-way FPN that aggregates the features in a top-down and bottom-up way, resulting in a semantically rich multiscale features. The semantic segmentation head uses the output of the FPN to perform segmentation using DPC and modules~\cite{mohan2021efficientps}. The instance information is extracted using a Mask-RCNN~\cite{he2017mask} head. And finally, the panoptic fusion head fuses the semantic and instance segmentations and outputs the panotic segmentation. This model has several advantageous including, the ability to control the backbone's complexity, a state-of-art results on Cityscapes~\cite{cordts2016cityscapes} benchmark. The code is easy to integrate, and it is open-sourced. This model was extended with depth, ego-pose and object pose information in will presented in Chapter~\ref{ch:ch4}.   

% A General advancement of that field 
% Explain in more details Panoptic Seg




\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{ch2/epsnet.pdf}
    \caption{Overview architecture of EfficientPS~\cite{mohan2021efficientps}. This model consists of a shared backbone with our 2-way FPN to extract features and parallel semantic and instance segmentation heads followed by our panoptic fusion module. Adopted from ~\cite{mohan2021efficientps}}
    \label{fig:panoptic-seg}
\end{figure}

\section{The transformer modules}

In the seminal work, Vaswani~\ea~\cite{Vaswani} have introduced the transformer. A neural network module that relies on attention to perform computation on sequences. Initially this module was intended for natural language processing (NLP), however, its success has shone in all data domains including, audio, image, video ...etc. This module has revolutionized the field, with great success in nearly all modalities and cross-modality tasks. In this section, we will first introduce the original transformers~\cite{Vaswani} and the image variation derived from it~\cite{liu2021swin,dosovitskiy2020}.

\subsection{Attention is all you need: the transformer}

Classical sequence modeling approaches used LSTMs and RNNs which processed data sequentially, where the current state $S_t$ was based on the previous state $S_{t-1}$ and an implicit memory that represents the past. This method had limitations as the current state did not have explicit access to all previous states and only relied on the implicit memory. Transformers were introduced to overcome this problem by using an attention mechanism. This allowed each state $S_i$ to pay attention to all other states based on their importance, determined by a weighting in the attention map. For example, in the sentence "A man walked into the park with his dog. He stopped to tie his shoe." the state "He" and "his" would pay more attention to "A man" as it is more relevant to these state.


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{ch2/trasnfomers.pdf}
    \caption{Overview of the transformer architecture. Figure adopted from~\cite{Vaswani}}
    \label{fig:vaswani}
\end{figure}



\reffig{vaswani} shows the architecture of the transformer. First, the text input is embedded into a continuous higher dimension. As the transformer is permutation invariant, explicit information of the embedding position should be added. A sinusoidal positional encoding is added to represent the position of each word. The first block of the transformer architecture is the \textit{encoder}. It processes the embedded and positional encoded input through a series of multi-head attention mechanisms, where each attention mechanism allows the model to attend to different parts of the input sequence and to weigh the importance of each part. The multi head attention is defined as:

First we constitute the Key, Query, Value as follows :
\begin{align}
    \text{Key: }   \mbf{K}  &= \mbf{X}\mbf{W_k} \\
    \text{Query: } \mbf{Q}  &= \mbf{X}\mbf{W_q} \\
    \text{Value: } \mbf{V}  &= \mbf{X}\mbf{W_v}
\end{align}
The multi head attention is defined as : 
\begin{align}
    \textbf{Attention} = \text{Softmax}(\frac{\mbf{Q}\mbf{K}^T}{\sqrt{d_{dim}}})\mbf{V}
\end{align}
The $\text{Softmax}(\frac{\mbf{Q}\mbf{K}^T}{\sqrt{d_{dim}}})$ produces an attention map normalized with the softmax that indicates the relative importance of the values with respect to each other. Thus, enabling the model to attend to the most relevant parts of the input. This hidden state is passed through a feedforward neural network to increase the complexity of the learned function. The skip connection allows better gradient flow. Finally, the output is normalized.

The second block of the transformer architecture is the \textit{decoder}, which generates a target sequence. Similar to the encoder, the decoder also uses multi-head attention mechanisms and feedforward neural networks. The difference is that the decoder uses the output of the encoder for the key and the value enabling cross attention. The final output of the decoder is then compared to the target sequence and the model is trained to minimize the difference between the two.

This architecture has several advantages as the attention is fully parallelizable and each state have access to all other states. However, the complexity of the attention grows quadratically with the sequence length $n$.
% The basic transfomer : 
% architecture
% equations
% complexitu
% It was introduced into vision 
\subsection{The Visual transformer (ViT)}
Applying directly, self-attention to images requires that each pixel attends to every other. This does not scale for realistic images, as the cost of the attention is quadratic in the number of pixels. To this end,~\cite{dosovitskiy2020image} marked the first transformer only architecture. The idea of this paper is instead of using each pixel as input to the standard transformer, the image is divided into small patches of $16\times16$ and the image will then be represented as a sequence of patches. 

\reffig{ViT} shows the architecture of ViT~\cite{dosovitskiy2020image}. The authors applied a standard
Transformer enocder~\cite{Vaswani} directly to images, with the fewest possible modifications. To do so, they split an image
into patches of $16\times16$. Image patches are treated the same way as tokens (words) in an NLP application. They provide this sequence of linear embeddings of these patches as an input to a Transformer. 

This architecture has known great success in the computer vision community. This backbone has been applied to nearly all tasks, replacing its CNN counterpart. The flexibility and the global receptive field of transformer enable the context-aware rich feature extraction. However, as the transformer is permutation  invariant and lacks the indicative bias of convolution networks (\ie the spatial information is hard-coded in the convolution filters. a $3\times3$ convolution is applied locally on a square of $3$), it is not able to obtain great results when trained on smaller datasets from scratch. 


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{ch2/model_scheme.pdf}
    \caption{Overview of the ViT architecture. Adopted from~\cite{dosovitskiy2020image}}
    \label{fig:ViT}
\end{figure}

\subsection{SwinTranformer (SwinT)}
In standard ViTs, the number of tokens and token feature dimension are kept fixed throughout different blocks of the network. This is limiting, since the
model is unable to capture fine spatial details at different scales. 
The Swin Transformer~\cite{liu2021swin} proposes a multi-stage hierarchical feature extraction that computes attention within a local window, by partitioning the window into multiple sub-patches. To capture interactions between different windows (image locations), window partitioning is gradually shifted, along the depth of the network, to capture overlapping regions

\reffig{swin} shows the architecture. Swin Transformer incorporates a shifted window approach for computing self-attention, as demonstrated in the accompanying illustration. In Layer l (on the left), a standard window partitioning strategy is used and self-attention is computed within each window. In the subsequent Layer l+1 (on the right), the window partitioning is shifted, leading to the creation of new windows. The self-attention computation in these new windows crosses the boundaries of the previous windows in Layer l, thereby establishing connections between the windows.


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{ch2/HiT-arch-v2.pdf}
    \caption{Overview of Swin tranformer architecture. Adopted from~\cite{liu2021swin}}
    \label{fig:swin-overview}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{ch2/HiT-layer2.pdf}
    \caption{Overview of Swin tranformer block. Adopted from~\cite{liu2021swin}}
    \label{fig:swin}
\end{figure}

\input{ch2/depth}


==> ch2/depth.tex <==

\section{Depth prediction}
\label{sec:background-depth}
The ability to perceive the 3D structure of the world is a fundamental aspect of human vision. It allows us to perceive the distance and relative position of objects in the world, as well as to judge the size, shape, and orientation of objects. One common use is in the field of robotics is autonomous driving (AD) and advanced driver-assistance system (ADAS), depth perception is used for path planing, automatic emergency braking (AEB), automatic cruise control (ACC) and many more. 
% add appilcation of Depth and the diffrent sensor  

The human brain is able to recognize the depth of the objects based on several clues that are present in the visual scene such as disparity, motion parallax, perspective, memorization, and shading. For example, the lateral separation of the eyes enables identifying an object from two angles, The brain uses this difference to compute the relative disparity. Motion parallax is the relative motion of objects at different distances as the viewer moves or the camera pans. The brain uses this motion to infer the depth of objects. 
%the prior knowledge about shapes could also help to infer the depth. A typical human for example is between 150 and 200 cm tall. Shading is the variation of brightness and color on an object due to the interaction of light with its surface and the surrounding environment. 

There are several sensors that can be used to measure depth, including:
\begin{itemize}
    \item \textbf{Stereoscopic cameras:} These use two cameras to capture images of the same scene from a slightly different position. The difference in the images can be used to calculate the depth of objects in the scene.
    %\item \textbf{LiDAR (Light Detection and Ranging)}: This involves emitting a laser light and measuring the time for the reflected light to return to the receiver.
    \item \textbf{Structured light:} This involves projecting a pattern of light onto a scene and using the distortion of the pattern to calculate the depth of objects in the scene.
    \item \textbf{Time-of-flight cameras}: These measure the time it takes for a pulse of light to travel from the camera to an object and back again, which can be used to calculate the distance to the object.
\end{itemize}





\subsection{Camera versus LiDAR for autonomous driving}
The use of cameras and LiDAR in autonomous driving is an ongoing topic of discussion among researchers and engineers. Although both technologies have their own advantages and disadvantages, the cameras are generally considered to be more affordable and versatile, while LiDAR is known for its superior accuracy and range.

LiDAR (Light Detection and Ranging) is an active 3D sensor that emits light to measure the distance to objects and provide a high-resolution 3D representation of the environment. LiDAR has become an increasingly popular technology in a wide range of applications such as autonomous vehicles due to its several advantages.

\begin{itemize}
    \item One of the main advantages of LiDAR is its high accuracy. Lidar can acquire high-precision data with a resolution of a few centimeters, making it suitable for applications that require precise measurements. In addition, LiDAR has a long range and can detect objects several kilometers away. This makes it useful in applications such as self-driving cars, localizing and mapping. Another advantage of LiDAR is its 3D imaging capabilities. LiDAR can produce real-time 3D point clouds of the environment, allowing for the creation of detailed 3D maps and models. Furthermore, LiDAR as active sensor can operate in any poor lighting conditions, making it useful for both day and nighttime applications. Despite its advantages, LiDAR has several disadvantages, the most notable being the cost, which can range from \euro$ 4,000$ to \euro$80,000$, making it less cost-effective than cameras. Additionally, LiDAR systems are weather sensitive and can be affected by conditions such as fog or rain, which can affect their accuracy and effectiveness. In addition, LiDAR systems consume a significant amount of power and are typically larger and heavier than cameras.

\end{itemize}

On the other hand, cameras are passive sensor that detect and measure the intensity of electromagnetic radiation, such as light. it consists of a lens to direct the incoming light and a light sensor to measure the intensity. Cameras have several advantages compared to LiDAR : 
\begin{itemize}
    \item The main advantages of cameras is their cost-effectiveness. They are widely available at a lower cost compared to LiDAR systems. Given the small margins in the automotive industry, the use of LiDAR is not practical and cameras are a more cost-effective sensor option. Cameras also have the added benefit of being able to perform multiple tasks, such as object detection, lane segmentation, and traffic sign recognition, making them a more attractive option for self-driving vehicles. Despite its advantages, cameras have some other limitations, including lighting conditions. Cameras can be affected by poor lighting conditions, which can make it harder to obtain accurate images. They also have a limited range, which means they can only detect objects within a certain distance. Using cameras for mapping can raise privacy concerns, particularly when they are used in public spaces.
\end{itemize}
Fusing LiDAR and camera modalities has proven to be an extremely effective approach for autonomous vehicles and other applications. The LiDAR sensor provides precise 3D spatial information, while the cameras provide high-resolution visual data. By using data from both modalities, it is possible to improve the accuracy and robustness of object detection, location, and tracking. In particular, LiDAR can provide accurate depth information and help detect objects in low light conditions or obscured by other objects. On the other hand, cameras can provide detailed visual information that can be used to detect objects and improve their identification. Furthermore, integrating both modalities reduces the disadvantages of each individual sensor, such as using LiDAR to detect objects in poor weather conditions and cameras to detect objects in optimal weather conditions. In summary, the fusion of LiDAR and camera data provides a more complete and accurate view of the environment, enabling the development of safer and more reliable autonomous systems.


\subsection{Classical methods for depth prediction}
In computer vision, depth perception has been studied extensively as a means of understanding and interpreting visual scenes. We could distinguish two approaches for depth prediction: monocular methods and multi-view methods 
\subsubsection{Classical methods for monocular depth prediction}
The depth is recovered from the motion of the camera. The scene is captured from different view and by knowing the relative position of camera it possible to recover the depth up to a certain scale. This algorithm is known as Structure from motion (SFM). Here is a typical structure from motion algorithm : 

\begin{enumerate}
    \item Load a set of images and detect keypoints and extract the descriptors (such as SIFT or ORB) for each image.
    \item Find correspondences between the keypoints of different images using descriptor matching.
    \item Estimate the fundamental matrix for each pair of images with correspondences.
    \item Compute the essential matrix for each pair of images.
    \item Use the essential matrix to compute the camera pose for each image.
    \item Triangulate the 3D positions of the corresponding points using the camera pose for each image.
\end{enumerate}



\subsubsection{Classical methods for multi-view depth prediction}
One example to perform multi-view depth prediction is stereo matching. It is a computer vision technique used to estimate the 3D structure of a scene from two or more images taken from different viewpoints. It involves finding corresponding points between the images and using these correspondences to compute the depth of each point in the scene.

There are many algorithms for stereo matching, but one of the most popular is the block matching algorithm. This algorithm works by dividing each image into small blocks, and then comparing the blocks from one image to the blocks in the other image to find the best match. The difference in position between the matching blocks is used to estimate the depth of the points in the scene. Here is a typical stereo matching algorithm : 
\begin{enumerate}
    \item Load two images of the same scene taken from different viewpoints.
    \item Rectify the images.
    \item Set the search window size and block size.
    \item For each block in the left image:
            \begin{enumerate}
            \item Search for the best matching block in the right image within the search window.
            \item Calculate the difference in position between the matching blocks.
            \item Use the difference in position to estimate the depth of the points in the block.
            \end{enumerate}
\item Repeat the process for each block in the right image.
\end{enumerate}


These classical methods are limited in their ability to handle complex and varied scenes, and are prone to errors and ambiguities. With the advent of deep learning, it has become possible to learn more robust and effective features for depth perception from large amounts of data. Instead of relying on hand-crafted features that may not encode relevant information for depth prediction. Deep learning approaches learn from the data the optimal features for depth prediction. These methods have achieved significant progress and outperform classical methods. 





\subsection{Deep learning for depth prediction}
In recent years, deep learning has emerged as a powerful tool in the field of depth prediction. This is due in large part to the success of convolutional neural networks (CNNs), which have surpassed other classical methods that rely on hand-crafted features. One of the key advantages of deep learning is its ability to learn features directly from data. This allows the model to automatically adapt to the task at hand and model complex situations, making it more powerful tool than traditional methods that relied on hand-crafted features.
Furthermore, CNNs have a hierarchical structure, which allows them to learn features at different levels of abstraction. This hierarchical structure is especially useful for depth prediction, as it allows the model to learn both low-level features, such as edges and textures, as well as high-level features, such as object shape and context.


\subsubsection{Depth prediction taxonomy}
Depth prediction is a challenging task that has been widely studied in the field of computer vision. One way to organize the various methods and models for depth prediction is through a taxonomy based on the input data or the supervision used \reffig{taxonomy-depth}.
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{ch2/tree_sota.pdf}
    \caption{Taxonomy of deep learning methods for depth prediction}
    \label{fig:taxonomy-depth}
\end{figure}
\subsubsection{Classification based on input data}
One way to classify the methods for depth prediction is based on the input data used. This includes:

\begin{itemize}
    \item \textbf{Monocular depth prediction:} uses a single image as input and estimates the depth information from it. By learning to infer object sizes and distinguish between foreground and background elements.
    \item \textbf{Stereo depth prediction:} uses two images captured from different viewpoints as input and estimates the depth information by comparing the two images. This is done by matching the two views and calculating the disparity between the images.
    
    \item \textbf{Multi-view depth prediction:} use multiple images captured from different viewpoints as input and estimate depth information by combining information from all the images. These methods have been shown to be effective in improving the performance of depth prediction on large-scale datasets. Multi-view depth prediction methods benefit from the strong epipolar geometry prior. This constraint provides additional information that can be used to improve the accuracy of depth prediction.

    \item \textbf{LiDAR completion:} LiDAR completion is a method that uses a partial depth map acquired by a LiDAR sensor as input and infers the missing depth information. LiDAR's sensors are known for their high accuracy and resolution, which makes them suitable for depth prediction. LiDAR's completion aim to generate a dense depth map from the sparse LiDAR map using camera information. 

\end{itemize}

Deep learning models perform best when provided with more information. Among the different methods for depth prediction, LiDAR completion has the lowest entropy (\ie provide the lowest uncertainty), as it already provides a sparse and accurate depth map that only needs to be completed. Multi-view systems come in second, as this method leverages more information and have a strong epipolar geometry constraint. On the other hand, monocular depth prediction has the highest entropy. This is because extracting 3D information from a single 2D image is an ill-posed problem. The scale of the objects in the scene is not known. Monocular depth prediction methods have to rely on other cues, such as texture, color, and motion, to estimate depth. These methods have the highest uncertainty and are prone to the scale ambiguity problem. However, the performance gap of these methods is closing and the prevalence of monocular cameras is making their applications more accessible and interesting. Another aspect to consider is the application: a monocular camera is found on all devices nowadays. Performing depth on these devices is more interesting as it enables a wide range of applications. 







\subsubsection{Classification based on learning}
Another way to classify depth prediction methods is based on the type of supervision used during training. This includes:

\begin{itemize}
    \item \textbf{Supervised depth prediction:} uses ground truth depth maps as the supervision during training. Supervised learning is the best-performing method for depth prediction in the benchmark, as it uses acquired depth maps obtained from depth sensors as supervision for the network. Assuming good accuracy of the ground-truth provided by depth sensors, these models have the best performance as the information provided for supervision is accurate and reliable. However, the use of ground-truth depth maps for supervision is not always feasible, as they can be expensive to acquire or unavailable. Furthermore, as the amount of the available labeled data is very limited, the generalization of these models are not guaranteed when deployed in complex environment.

    
    \item \textbf{Self-supervised depth prediction:} these methods have been proposed as an alternative to supervised methods. These methods use a differentiable warping to reconstruct a set of a source images (monocular video, stereo video …etc.) into a target images. This is done using a depth network and pose a network when the pose is not known (\eg the case of monocular video). These models are very practical as they can be easily trained, as they only require a video as input. The data is cheap to collect and widely available, as billions of videos are already available on platforms such as YouTube.


    \item \textbf{Semi-supervised depth prediction:}  proposed as a solution that combines the advantages of both supervised and self-supervised methods. These models use a combination of ground-truth depth maps and other forms of supervision, such as depth estimates from self-supervised methods or depth priors. These methods have been shown to be effective in improving the performance of depth prediction on large-scale datasets, while also being more practical as they do not require ground-truth depth maps for all the data.
\end{itemize}


The state-of-art of depth prediction will be discussed further in Chapter~\ref{ch:ch3}

==> ch3/depth.tex <==
In this chapter, the primary objective is to explore and analyze the different methodologies that are utilized for depth prediction. The discussion begins by delving into the advantages and benefits of self-supervised learning. First, the highlight will be focused on self-supervised learning. This method allows leveraging unlabeled data, which is typically more abundant and less costly to obtain than labeled data, making it a more practical option in some cases.
Afterward, an overview of the literature on supervised learning, which includes a detailed description of various supervised methods that have been developed for depth prediction. These methods leverage labeled data, and while they are often considered the gold standard for achieving high accuracy, they come with their own set of limitations. One major challenge associated with supervised learning is the difficulty in obtaining labeled data, as it can be time-consuming, costly, and in some cases, impractical. In addition, as supervised methods rely on labeled-dataset they can be prone to overfitting and bias, which limits their ability to generalize to unseen data. for that end,  a novel approach called the acontrario GAN method is proposed. This method aims to enhance generalization in supervised learning.
In the latter part of the chapter, the attention is shifted towards self-supervised learning for depth prediction and provide a comprehensive overview of this methodology. We cover the problem formulation, how self-supervision is performed, and related literature.















\section{Supervised versus self-supervised approaches}
% SUperivsed learning
In recent years, the field of deep learning has known a tremendous an exponential growth that has revolutionized the field of artificial intelligence. Since the unprecedented success of deep learning methods on the ImageNet~\cite{deng2009imagenet}, a plethora of expert models that can learn from massive amounts of labeled data were developed. Since then, there has been a rapid evolution of these models that have demonstrated impressive performance on a wide range of tasks.
However, the performance and generalization of these models are heavily dependent on the quality, quantity, and diversity of the training data. 


As illustrated in~\reffig{labled_unlabled}, the size of labeled dataset represent only a tiny portion of the unlabeled dataset, which in turn represent a tiny portion of the real world. Training only on the labeled dataset, yields models that are overly specialized, producing models that are susceptible to poor generalization. Furthermore, even if the model can successfully extrapolate beyond the labeled dataset, it will still only represent a small fraction of the possible scenarios that exist in the real world. Consequently, a model trained only on the labeled datasets is likely to suffer from biases, domain shifts, and poor generalization when confronted with extreme scenarios that were not part of the training dataset. 

\begin{figure}
    \centering
    \includegraphics[width=0.75\textwidth]{ch3/dataset.pdf}
    \caption{The size of labeled dataset represent only a tiny portion of the unlabeled dataset, which in turn represent portion of the real world}
    \label{fig:labled_unlabled}
\end{figure}


Despite the remarkable success of supervised learning in deep learning, there are limitations to the extent that AI can progress solely based on this approach. One of the most significant challenges facing supervised learning is the difficulty of obtaining and labeling large amounts of data, especially for real-world problems that are complex and diverse, such as autonomous driving applications. This obstacle necessitates the development of alternative approaches that can learn from directly from unlabeled data. Labeling everything is just impossible.

One inspiration to learn without labels is the human intelligence. We have the ability to learn directly through observation: Human beings possess the ability to formulate hypotheses based on our experiences, conduct experiments to test these hypotheses, observe the results, and ultimately derive logically-sound conclusions. Similarly, we could also make machines learn solely from the data, where the learning obtains the supervisory signals from experience,\ie data, only. This is known as self-supervision. One good example that illustrates the potential of these methods is  the GPT~\cite{openai2023gpt4} family. These models have been trained to predict the next token (word or image patch) in a sequence, leveraging a huge dataset of text crawled from the internet, arXiv papers, and books. These self-supervised  models have shown impressive results. They can even outperform supervised models on several tasks with zero-shot (without being trained explicitly to perform these tasks). Furthermore, some results suggest that the quality of self-supervised representations increase logarithmically in proportion to the volume of unlabeled pretraining data used~\cite{goyal2019scaling}. This means that the performance may advance over time as advances in computational capacity and data acquisition enable ever-larger datasets to be utilized without the necessity of manually labeling new data. 


The following sections will first introduce depth prediction using supervised methods. The self-supervised methods will be introduced after. Finally, A discussion of the advantageous and drawbacks of each approach is developed. 

\section{Depth prediction with supervised methods}
The supervised approach relies on acquired depth maps obtained from depth sensors such as LiDAR as the supervision signal for the network. These methods have achieved good results on the benchmarks.

\subsection{Problem formulation}
Depth prediction from RGB images using supervised learning can be viewed as a regression problem. Given an RGB image (multiple images in the case of stereo or MVS), $\mbf{I}$, and a corresponding depth map, $\mbf{D}$, the goal is to learn a mapping function with the set of parameters $\bm\theta$, $\mbf{D} = f(\mbf{I}, \bm\theta)$, between the image and the depth map using a training dataset, $T$, consisting of image-depth pairs $(\mbf{I}_i, \mbf{D}_i)$. A convolutional neural network (CNN) could be trained to perform this task, with a basic architecture consisting of an encoder and a decoder. The encoder extracts abstract information from the image using sequential convolutional blocks, while the decoder uses up-sampling modules to increase the resolution of the depth map. Usually these models are supervised using L1, L2, scale-invariant errors or Huber loss for a robust optimization. 
\begin{itemize}
    \item L1 loss : 
    \begin{align}
    L1 = \frac{1}{N} \sum_{i=0}^{N}|\mbf{D}^i - \mbf{D_{gt}^i}|
    \end{align}
    
    \item L2 loss : 
    \begin{align}
    L2 = \frac{1}{N} \sum_{i=0}^{N}||\mbf{D}^i - \mbf{D_{gt}^i}||^2
    \end{align}
    
    \item Huber loss : 
    \begin{align}
       \text{Huber} = \frac{1}{N} \sum_{i=0}^{N} \begin{cases} \frac{1}{2} (\mbf{D}^i - \mbf{D_{gt}^i})^2 & |\mbf{D}^i - \mbf{D_{gt}^i}| \leq \delta \\ \delta (|\mbf{D}^i - \mbf{D_{gt}^i}| - \frac{1}{2} \delta) & \text{otherwise} \end{cases}   
    \end{align}
    \item Scale invarient loss :
        \begin{align}
            \text{Scale inv} = \frac{1}{2N} \sum_{i=0}^{N} \Big( \log(\mbf{D}^i) - \log(\mbf{D_{gt}^i}) + \frac{1}{N} \sum_{i=0}^{N} \big( \log(\mbf{D}^i) - \log(\mbf{D_{gt}^i}) \big) \Big)
        \end{align}
\end{itemize}
\subsection{Monocular methods}
Eigen~\cite{Eigen2014}~\ea were among the first to investigate using deep learning for depth inference and developed a CNN network with two deep stacks. \reffig{eigen-arxh} shows the architecture. The first stack was used for preparing the input image and refining the depth map, the second stack was responsible for arranging the obtained coarse depth predictions with the objects in the scene.
\begin{figure}
    \centering
    \includegraphics[width=0.75\textwidth]{ch2/arch_vertical.pdf}
    \caption{Architecture for Eigen~\ea~\cite{Eigen2014}. Using a single image as input, the depth is reconstructed. The first stack was used for preparing the input image and refining the depth map, the second stack was responsible for arranging the obtained coarse depth predictions with the objects in the scene. Adopted from~\cite{Eigen2014}}
    \label{fig:eigen-arxh}
\end{figure}
This approach has led to an increased focus on convolutional architectures for depth prediction, with methods such as CLIFFNet~\cite{Wang2020} and Transformer-based networks like TransDepth~\cite{Zhao2021} and DPT~\cite{Ranftl2021}. These methods propose to replace convolution operations with Transformer layers, which further improve model performance. However, these methods have faced challenges with slow convergence and suboptimal solutions. Another approach to depth prediction involves discretizing continuous depth and treating it as a per-pixel classification problem. Methods like DORN~\cite{Fu2018}, which uses an ordinal classification depth estimation loss and an ASPP module~\cite{chen2017deeplab} to extract multi-level information, and Adabins\cite{Bhat2021}, which uses an adaptive bin's strategy to further improve the model performance. BinsFormer~\cite{Li2022} proposes classification-regression-based monocular depth estimation that utilizes Transformer layers for adaptive bin generation and a multiscale refinement strategy. 

\subsection{Stereo methods}
The field of stereo matching has undergone significant advancements in recent years, owing to the incorporation of deep learning techniques. Early works in this domain primarily focused on the use of Siamese networks for extracting patch-wise features or predicting matching costs~\cite{Luo2016,Zagoruyko2015,Zbontar2015}. Using end-to-end networks, researchers have been able to achieve more accurate results by jointly learning all steps of the stereo matching process~\cite{Shaked2017,Song2021}. Another line of research is the use of cost volume layer~\cite{Kendall2017}, which enables the network to perform per-pixel feature matching.
To improve the computational efficiency of stereo matching, researchers have proposed cascaded models~\cite{Pang2017,Yang2019,gidaris2017detect} that perform the search in disparity space in a coarse-to-fine fashion. In particular, the method proposed in~\cite{Pang2017} utilizes multiple residual blocks to improve the current disparity estimate. A more recent work~\cite{yang2019hierarchical} relies on a hierarchical cost volume, which allows the method to be trained on high-resolution images and generate different resolutions on demand.~\cite{tankovich2021hitnet} is inspired by classical stereo matching methods, it proposes an end-to-end learning approach that overcomes the issues of hand-crafted algorithms, while maintaining computational efficiency as it does not explicitly build a volume, and instead it relies on a fast multi-resolution initialization step, differentiable 2D geometric propagation and warping mechanisms to infer disparity hypotheses.
\subsection{Multi-view stereo (MVS)}
Multi-view stereo (MVS) addresses dense 3D representation using a series of calibrated images with known poses. Typically, a MVS network extracts image features by a CNN and constructs cost volume via plane sweep algorithm in which source images are warped to the reference view.~\cite{Yao2018} proposed MVSNet, which utilizes a 2D CNN to extract features and a 3D CNN for cost regularization in order to infer depth maps for large-scale MVS reconstruction. To address the high memory consumption of the 3D CNN, the cost volume is regularized with gated recurrent units (GRUs) in~\cite{Yao2019}. Additionally, Wei \ea~\cite{Wei2021}. proposed AA-RMVSNet, which employs adaptive aggregation and long short-term memory (LSTM) to further improve the performance of MVS reconstruction. Fast-MVSNet~\cite{yu2020fast}, was the first to propose a sparse cost volume to infer an initial sparse depth map and then optimizes the sparse depth map gradually.~\cite{Gu2020} constructed a cascade cost volume in a coarse-to-fine manner to recover a high-resolution depth map. \cite{Cheng2020} built adaptive thin volumes in multiple stages to progressively increase depth resolution and precision. Furthermore,~\cite{Yang2022} designed CVP-MVSNet, which utilizes a pyramid structure to iteratively refine depth maps.~\cite{Wang2021} introduced the traditional patchmatch stereo algorithm into a learning-based coarse-to-fine framework. While these learning-based methods have achieved significant success, they still face challenges such as match ambiguities and mismatches in challenging regions, likely due to insufficient global context and 3D-inconsistent representations.











\subsection{The generalization of supervised approaches}
As supervised methods rely on labeled datasets, the generalization of these models could be limited. Most of the benchmarks are predominately daytime and do not include complex situations such as weather variations. We have explored the possibility of using GANs in order to improve the generalization of the supervised method. Several works were proposed in the literature to improve the generalization using GANs, this includes applications such as domain adaptation~\cite{Kim2019,Sankaranarayanan2018,Yang2020,Vu2019}. \cite{porav2019don} leverage CycleGAN~\cite{zhu2017unpaired} to create a multi-domain labeled dataset. By translating a labeled daytime dataset into nighttime style. These images will be used to perform domain adaptation. Similarly, we have proposed to train an end-to-end model that performs at the same time style-transfer and domain adaptation~\cite{boulahbal:hal-03365983}. However, A fundamental problem with generative models is \textbf{hallucination}. These models tend to create outputs that are not consistent with the conditioning input variable. This could be problematic in domain adaptation. We have investigated this problem further, and we have discovered that the classical conditional GAN approach applied to these models is not fully conditional, and the discriminator does not learn this property of the data (\ie the conditionality). More information about the problem, the formulation, the validation protocol, and the results are presented in Appendix~\ref{ch:apdx}. In the following, we present the method and results of the \textit{acontario cGAN} on a depth prediction problem.   

\subsubsection{Classic cGAN}
\label{sec:ccgan}

Classical cGAN training is based on conditionally paired sets of data $\mathcal{C}(\mbf{x},\mbf{y})$ where $\mbf{x}\sim p(\mbf{x})$ is the condition variable and $\mbf{y}\sim p(\mbf{y}|\mbf{x})$ is the real training variable. The generator of a cGAN outputs a transformed set of data $\mathcal{C}_G(\mbf{x},\mbf{y}_G)$ composed of the generator output variable $\mbf{y}_G\sim p_G(\mbf{y})$ and the condition variable. These sets of data will be called "real-conditional" and "generated-conditional" respectively. 
The discriminator is defined as:
\begin{align}
    D(\mbf{x},\mbf{y}):=\mathcal{A}(f(\mbf{x},\mbf{y}))
    \label{eq:discriminator}
\end{align}
Where $f(.)$ is a neural network function of $\mbf{x}$ and $\mbf{y}$, and $\mathcal{A}$ is the activation function whose choice depends on the objective function. The classical cGAN objective function is defined as: 
\begin{align}
         \mathcal{L}_{adv}= \min_{G} \max_{D} \left(\: \mathbb{E}_{\mbf{x}\sim p(\mbf{x}),\mbf{y}\sim p(\mbf{y}|\mbf{x})}\big[log(D(\mbf{x},\mbf{y})]\big] +   \mathbb{E}_{\mbf{x}\sim p(\mbf{x})}\big[log[1 - D(\mbf{x},G(\mbf{x}))]\big] \right)
\label{eq:classic_loss}
\end{align}
The min-max activation function is defined as a Sigmoid $\mathcal{A}(\mbf{x})=\left({\frac{1}{1+e^{-\mbf{x}}}}\right)$.




\subsubsection{Acontrario conditionality loss}
\label{sec:consistency}




The proposed \ac cGAN approach~\cite{Boulahbal2021BMVC} is based on training with unconditionally paired sets of data, obtained by randomly shuffling or paring the original conditional sets of data. The \ac set is defined as $\mathcal{C}_U(\mbf{\tilde x},\mbf{y})$, where $\mbf{\tilde x}\sim p(\mbf{x})$ is the \ac conditional variable ($\mbf{\tilde x} \neq \mbf{x}$) and $\mbf{y}$ is the real training variable as in Section~\ref{sec:ccgan}. In this case $\mbf{\tilde x}$ and $\mbf{y}$ are independent. The generator of the \ac cGAN outputs a transformed set of data $\mathcal{C}_{UG}(\mbf{\tilde x},\mbf{y})$ composed of the generator output variable $\mbf{y}_G\sim p_G(\mbf{y})$ and the random variable $\mbf{\tilde x}$. These two sets of data will be called "real-\ac" and "generated-\act" respectively. The motivation to create these new sets is to train the discriminator to correctly classify unconditional data as false. Figure~\ref{fig:pipeline} shows the four possible pairings. In practice, random sampling of \ac pairs is carried out without replacement and attention is paid to not include any conditional variables into a same batch while processing.

In order to enforce conditionality between $\mbf{y}$ and $\mbf{x}$ an \ac term is proposed as:
\begin{align}
        \mathcal{L}_{ac}= \max_{D} \: & \left(\mathbb{E}_{\mbf{\tilde x} \sim p(\mbf{\tilde x}) ,\mbf{y}\sim p(\mbf{y})}\big[log(1 - D(\mbf{\tilde x},\mbf{y}))\big]  + 
        \mathbb{E}_{\mbf{\tilde x} \sim p(\mbf{\tilde x}) ,\mbf{x} \sim p(\mbf{x})}\big[log(1 - D(\mbf{\tilde x},G(\mbf{x})))\big] \right)
\label{eq:ac_loss}
\end{align}
The first term enforces the real-\act pairs to be classified as false. The second term enforces the generated-\act as false. The final loss is:
\begin{align}
    \mathcal{L}_{adv}^{'}  = \mathcal{L}_{adv}+ \mathcal{L}_{ac}
\label{eq:overall_loss}
\end{align}

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{ch3/im-to-depth.pdf}
    \caption{Qualitative results for depth prediction. The \ac cGAN shows better performance and more consistent prediction with respect to the input. The first row shows a case of mode collapse for the baseline as it ignores completely the input.}
    \label{fig:depth_qualitative}
\end{figure*}






\subsubsection{Experiement results}






























\section{Depth prediction with self-supervised methods}
\label{sec:ssl}

Self-supervised depth prediction refers to methods that only use images for input and supervision, without the need for ground-truth labels. These methods are becoming increasingly popular due to their practicality, as they do not require manually labeled training data. 
\subsection{Problem formulation}
The aim of monocular depth prediction is to learn an accurate depth map through the mapping $\mbf{D}_t = f(\img{t-k:t}; \bm{\theta})$ where $\img{t-k:t} \in \mathbb{R}^{k \times W\times H\times3}$ is $k$ context images. $\mbf{D}_t$ is the target depth. $\bm{\theta}$ are the network parameters.  
In self-supervised learning, this model is trained via novel view synthesis by reverse warping a set of source frames $\mbf{I}_{s}$ into the target frame $\mbf{I}_{t}$ using the learned depth $\mbf{D}_{t}$ and the target to source pose $\pose{s}{t} \in \mathbb{SE}[3]$. The reverse warping $\mathcal{W}$ is used to reconstruct the image. It involves mapping pixels from one image to another image, where the pixel coordinates in the new image are computed based on the differentiable warping function applied to the original image the mapping is defined as: 
\begin{equation}
        \label{eq:warping_classic}
        \widehat{\pt}_{s} \sim \mbf{K} \pose{s}{t} \mbf{D}_{t}  \mbf{K}^{-1} \pt_{t}
\end{equation}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{ch2/Photometric_loss.pdf}
    \caption{An illustration of the reverse (also called inverse) warping. Using the depth and the pose, the source image is warped into the target image. The self-supervised optimization is done using the photometric loss.}
    \label{fig:inver-warping}
\end{figure}
The image is reconstructed using the interpolation.~\reffig{inver-warping}~\refeq{warping_classic} shows the warping process. The points of the target image are back-projected using the camera parameters and the learned depth. The $\pose{s}{t}$ is applied to transform the point cloud. Finally, the point cloud is projected using the camera parameters. The target image is obtained using the interpolation. Therefore, by knowing the depth and pose, the mapping from the image $\mbf{I}_{s}$ is used to reconstruct $\Hat{\mbf{I}}_t$ through a bi-linear interpolation.

\reffig{training-vs-test} Shows the pipeline for self-supervised monocular depth prediction. During training, the forward pass is propagated through the depth network and the pose network. The output of these networks will then be used to reverse warp a source image to reconstruct the target image. The photometric loss is calculated and the backward pass optimize both depth and pose network parameter simultaneously. At test-time, \textbf{only the depth network }is used and the pose network, unless used to reconstruct the image, it is discarded.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{ch3/SFM.pdf}
    \caption{Training-time versus test-time for self-supervised depth prediction. The red arrow shows the test-time pipeline, while the blue arrows show the training-time pipeline. The warping function and the pose network are used only during training.}
    \label{fig:training-vs-test}
\end{figure}


\subsection{Loss functions}
\label{sec:loss_function_ch3}
Let $\mathcal{L}$ be the objective function. The self-supervised setting casts the depth learning problem to an image reconstruction problem through the reverse warping. Thus, learning the parameters $\bm{\theta}$ involves learning $\widehat{\bm{\theta}} \in \bm{\Theta}$ that minimizes the following objective functions:
\begin{equation}
    \widehat{\bm{\theta}} = \argmin_{\bm{\theta} \in \bm{\Theta}} \frac{1}{n} \sum_{n} \mathcal{L} (f(\mbf{I}_t, \widehat{\mbf{I}}_t;\bm{\theta}))
    \label{eq:risk_minimzation}
\end{equation}
where $n$ is the number of training examples. There are several surrogate loss functions proposed to supervise the depth though image reconstruction, some of these losses are :
\begin{itemize}
    \item \textbf{Photometric loss: }
    
    Following~\cite{Zhou2017,Godard2019,Rares2020}, the photometric loss seeks to reconstruct the target image by warping the source images using the static/dynamic pose and depth. The $L_1$ loss is defined as follows:
    \begin{equation}
        \mathcal{L}_{rec}(\img{t}, \widehat{\mbf{I}}_{t}) = \sum_{\pt} | \img{t}(\pt) - \widehat{\mbf{I}}_{t}(\pt) |
    \end{equation}
    where $\widehat{\mbf{I}}_{t}(\pt)$ is the reverse warped target image obtained by~\refeq{warping_classic}. The L1 loss is a widely used loss function in computer vision tasks, and it is particularly useful for self-supervised depth prediction because it is robust to outliers. However, the L1 loss alone is not sufficient, as it does not take into account the structural similarity between the predicted image map and the ground-truth image.  

    \item \textbf{SSIM (Structural Similarity Index) }is used to improve the photometric loss for self-supervised depth prediction models. SSIM is a widely used metric for image quality assessment, and it measures the structural similarity between two images by comparing the luminance, contrast, and structure of the images. SSIM is particularly useful for self-supervised depth prediction because it is more sensitive to changes in the structure of the images than the L1 loss.
    
    Threfore, the photometric loss is defined as:
    \begin{equation}
    \begin{aligned}
      \mathcal{L}_\textup{pe}(\img{t}, \widehat{\mbf{I}}_{t}) = \sum_{\pt} \big[&(1 - \alpha) \textup{ SSIM}[ \img{t}(\pt) - \widehat{\mbf{I}}_{t}(\pt)]  \\
      & +  \alpha | \img{t}(\pt) - \widehat{\mbf{I}}_{t}(\pt) |\big]
    \end{aligned}
    \label{eq:ssim}
    \end{equation}
    \item \textbf{Depth smoothness: } An edge-aware gradient smoothness constraint is used to regularize the photometric loss. The depth map is constrained to be locally smooth through the use of an image-edge weighted $L_1$ penalty, as discontinuities often occur at image gradients. This regularization is defined as~\cite{heise2013pm}:
    \begin{equation}
    \begin{aligned}
      \mathcal{L}_{s}(D_{t}) = \sum_{p} \big[ &| \partial_x D_{t}(\pt) | e^{-|\partial_x \mbf{I}_{t}(\pt)|}    +\\
      &| \partial_y D_{t}(\pt) | e^{-|\partial_y \mbf{I}_{t}(\pt)|} \big] 
    \end{aligned}\label{eq:loss-disp-smoothness}
\end{equation}
\end{itemize}
In practice, to optimize the self-supervised depth prediction network, often, a L1 loss is used in combination with the SSIM and depth smoothness losses. This yields better results than using a single loss function alone.


\subsection{Monocular methods}
Depth prediction has been successful with self-supervised learning from videos. The seminal work of Zhou \ea~\cite{Zhou2017} introduced the core idea to jointly optimize the pose and depth network using image reconstruction and a photometric loss.~\reffig{zhou-method} To account for the ill-posed nature of this task, several works have addressed different challenges.~\cite{Vijayanarasimhan,xu2021moving,luo2019every} addressed the rigid scene assumption using optical flow and motion clustering.~\cite{Gordon2019,Shu2020} proposed more robust image reconstruction losses to reject the outliers such as occlusion during training.~\cite{chen2019self} addressed learning the camera parameters for better generalization.~\cite{Bian2019,Chen2019,Rares2020,Wang2021} addressed the scale ambiguity problem and propose to enforce depth scale and structure consistency.~\cite{mccraith2020monocular, Watson2021} employed a test-time refinement by allowing the model parameters to vary dynamically during inference using a photometric loss.

%~\cite{Klingner2020,Yin2018,Ranjan2019,Chen2019}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{ch2/method.pdf}
    \caption{The supervision pipeline for view synthesis is composed of two networks: the depth network and the pose network. The depth network uses only the target view as input to generate a per-pixel depth map. The pose network inputs both the target view and nearby/source views, and outputs the relative camera poses. These outputs are used to reconstruct the target view through reverse warping of the source views, and the reconstruction loss is used to train the CNNs in an unsupervised manner using videos as data. Adopted from~\cite{Zhou2017}}.
    \label{fig:zhou-method}
\end{figure}

\subsection{Stereo methods}
These models leverage a binocular video in order to supervise the network. These models have several advantageous over monocular methods: the pose transformation between left and right camera pair is constant. This pose could be estimated using camera calibration before acquiring the data. The pair captures the scene simultaneously (with infinitesimal time delay), this makes the observation of the scene from the stereo pair static. furthermore, the problem of occlusion is handled better as there is more spatial and temporal context to be used to handle occlusion. Several methods were proposed in the literature\cite{Wang2022,Peng2021,Bello2021,Zhu2020,Watson2019,Pilzer2019,Godard2017,Garg2016}.~\cite{Garg2016} was the first to propose a differentiable warping that warps the left image into the right and vice versa.~\cite{Godard2017} proposes single image depth estimation using binocular stereo input. This paper proposes a novel training objective function that enforces consistency between the disparities produced relative to both left and right images.~\cite{Pilzer2019} proposes a distillation method using teacher/student networks. This method computes the inconsistencies between input and cycle-reconstructed images and exploits them to generate state-of-the-art depth predictions through a refinement network.~\cite{Watson2019} addresses the local minima problem of photometric loss in self-supervision by incorporating depth suggestions from off-the-shelf stereo algorithms.~\cite{Wang2022} proposes a novel depth representation called PlaneDepth, which uses orthogonal planes, to estimate depth distribution using a Laplacian Mixture Model. The approach addresses the problem of discontinuity caused by near frontal-parallel planes and boosts the robustness of the representation for occlusions. 

\subsection{MVS methods}
The first unsupervised MVS framework that utilizes end-to-end learning is proposed by UnsupMVS~\cite{khot2019learning}. In this framework, the source view images are reversely warped to the reference view using a predicted depth map. JDACS~\cite{xu2021self} enforces cross-view consistency of extracted semantic features and utilizes non-negative matrix factorization to supervise the segmentation map. However, this approach still requires a pre-trained semantic feature extraction backbone and suffers from unstable convergence of cross-view semantic consistency, leading to unreliable supervision. U-MVSNet~\cite{xu2021digging} improves the supervision by employing a flow-depth consistency loss to generate pseudo labels for uncertainty-aware consistency, but it cannot be trained end-to-end and requires complex pre-training and fine-tuning. Self-supervised CVP-MVSNet~\cite{yang2021self} learns depth pseudo labels with unsupervised pre-training, followed by iterative self-supervised training to refine the pseudo label. However, it is still affected by ambiguous supervision. Moreover, these unsupervised and self-supervised methods lack an occlusion-aware module, leading to incomplete reconstruction of point clouds from different viewing directions. RC-MVSNet~\cite{chang2022rc} uses neural rendering to alleviate occlusions and non-Lambertian surfaces. It includes a depth rendering consistency loss to constrain geometry features close to the object surface and a reference view synthesis loss to provide consistent supervision.


\subsection{Discussion of self-supervised versus supervised monocular depth prediction approaches}



~\reftab{ssl-vs-sup} shows the comparison between self-supervised and supervised depth prediction methods on the KITTI benchmark~\cite{Geiger2012CVPR}, the supervised approaches represent the state-of-the-art in depth prediction tasks, yielding higher accuracy compared to SSL methods. Despite this observation, it is important to note that this comparison may not fully reflect the potential of SSL methods in depth prediction.

Self-Supervised Learning (SSL) methods offer a compelling advantage in training depth prediction models on large-scale datasets without the need for depth annotations. Unlike supervised methods, which heavily rely on annotated labels, SSL methods can leverage abundant unlabeled data to achieve high accuracy and overcome scalability limitations. By designing effective pretext tasks, such as image warping, SSL methods capture the structure and semantics of the data. The quality of self-supervised representations has been observed to improve logarithmically~\cite{goyal2019scaling} with the volume of unlabeled pretraining data, highlighting the vast potential of SSL methods in depth prediction tasks. This means that eventually, if SSL methods were trained on enough large scale datasets, these methods will surpass the supervised method. Furthermore, advancements in pretext tasks and model architectures for SSL can lead to even more accurate and robust depth predictions.

Therefore, it is important to consider the limitations of comparing self-supervised methods and supervised methods solely on a single dataset, such as KITTI. Such comparisons might not fully explore the capabilities of SSL methods, as they are confined to training on a specific dataset.





\begin{table*}
\centering
\footnotesize
\begin{tabular}{|c|l ||c c c c ||c c c|}
\hline
Approach & Method & Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline
Supervised 
 & Eigen~\cite{Eigen2014} & 0.203 & 1.548 & 0.282 & 6.307 & 0.702 & 0.898 & 0.967 \\
 & Kuznietsov et al~\cite{kuznietsov2017semi} & 0.113 & 0.741 & 4.621 & 0.189 & 0.862 & 0.960 & 0.986 \\
  & DORN~\cite{Fu2018} & 0.072  & 0.307 & 2.727 & 0.120 & 0.932 & 0.984 & 0.994 \\
 & TransDepth~\cite{Zhao2021} & 0.064 & 0.252 & 2.755 &  0.098 & 0.956 & 0.994 & 0.999 \\
 & DPT~\cite{Ranftl2021}  & 0.062 & –& 2.573 & 0.092 & 0.959 & 0.995 & 0.999 \\
 &Adabins~\cite{Bhat2021} & 0.058 & 0.190 & 2.360 & 0.088 & 0.964 & 0.995 &  0.999 \\
&BinsFormer~\cite{Li2022} &0.052 & 0.151 & 2.098 & 0.079 & 0.974 & 0.997 & 0.999 \\

       
\hline  
Self-supervised &
SfMlearner~\cite{Zhou2017}  & 0.183 & 1.595 & 6.709 & 0.270 & 0.734& 0.902 &0.959 \\
&Monodepth2~\cite{Godard2019}  & 0.115 & 0.903 & 4.863 & 0.193 & 0.877 & 0.959 & 0.981\\
&Lee \ea~\cite{lee2021attentive}  &  0.113 & 0.835 & 4.693 & 0.191 & 0.879 & 0.961 & 0.981 \\
&SGDepth~\cite{Klingner2020}  & 0.113 & 0.835 & 4.693 & 0.191 & 0.879 & 0.961 & 0.981\\
&SAFENet~\cite{lou2020safenet}& 0.112 & 0.788 & 4.582 & 0.187 & 0.878 & 0.963 & 0.983 \\
&Insta-DM~\cite{lee2021learning}& 0.112& 0.777 &4.772 &0.191& 0.872& 0.959& 0.982 \\
&PackNetSfm~\cite{Rares2020} & 0.111 & 0.785 & 4.601 & 0.189 & 0.878 & 0.960 & 0.982\\
&MonoDepthSeg~\cite{safadoust2021self} & 0.110 & 0.792 & 4.700 & 0.189 & 0.881 & 0.960 & 0.982 \\
&Johnston \ea~\cite{johnston2020self}  & 0.106 & 0.861 & 4.699 & 0.185 & \underline{0.889} & 0.962 & 0.982 \\
&Manydepth~\cite{Watson2021}  & 0.098 & 0.770 & 4.459 & 0.176 & 0.900 & 0.965 & 0.983 \\
\hline
\end{tabular}
\caption{Quantitative performance comparison of on the KITTI benchmark with Eigen split~\cite{Geiger2012CVPR}. For Abs Rel, Sq Rel, RMSE and RMSE log lower is better, and for $\delta < 1.25$, $\delta < 1.25^2$ and $\delta < 1.25^3$ higher is better.}
\label{tab:ssl-vs-sup}
\end{table*}





==> ch3_reformulated/depth.tex <==
In this chapter, the primary objective is to explore and analyze the different methodologies that are utilized for depth prediction. 

Afterward, an overview of the literature on supervised learning, which includes a detailed description of various supervised methods that have been developed for depth prediction. These methods leverage labeled data, and while they are often considered the gold standard for achieving high accuracy, they come with their own set of limitations. One major challenge associated with supervised learning is the difficulty in obtaining labeled data, as it can be time-consuming, costly, and in some cases, impractical. In addition, as supervised methods rely on labeled-dataset they can be prone to overfitting and bias, which limits their ability to generalize to unseen data. for that end,  a novel approach called the acontrario GAN method is proposed. This method aims to enhance generalization in supervised learning.
In the latter part of the chapter, 


















The following sections will first introduce depth prediction using supervised methods. The self-supervised methods will be introduced after. Finally, A discussion of the advantageous and drawbacks of each approach is developed. 

\section{Depth prediction with supervised methods}
The supervised approach relies on acquired depth maps obtained from depth sensors such as LiDAR as the supervision signal for the network. These methods have achieved good results on the benchmarks.

\subsection{Problem formulation}
Depth prediction from RGB images using supervised learning can be viewed as a regression problem. Given an RGB image (multiple images in the case of stereo or MVS), $\mbf{I}$, and a corresponding depth map, $\mbf{D}$, the goal is to learn a mapping function with the set of parameters $\bm\theta$, $\mbf{D} = f(\mbf{I}, \bm\theta)$, between the image and the depth map using a training dataset, $T$, consisting of image-depth pairs $(\mbf{I}_i, \mbf{D}_i)$. A convolutional neural network (CNN) could be trained to perform this task, with a basic architecture consisting of an encoder and a decoder. The encoder extracts abstract information from the image using sequential convolutional blocks, while the decoder uses up-sampling modules to increase the resolution of the depth map. Usually these models are supervised using L1, L2, scale-invariant errors or Huber loss for a robust optimization. 
\begin{itemize}
    \item L1 loss : 
    \begin{align}
    L1 = \frac{1}{N} \sum_{i=0}^{N}|\mbf{D}^i - \mbf{D_{gt}^i}|
    \end{align}
    
    \item L2 loss : 
    \begin{align}
    L2 = \frac{1}{N} \sum_{i=0}^{N}||\mbf{D}^i - \mbf{D_{gt}^i}||^2
    \end{align}
    
    \item Huber loss : 
    \begin{align}
       \text{Huber} = \frac{1}{N} \sum_{i=0}^{N} \begin{cases} \frac{1}{2} (\mbf{D}^i - \mbf{D_{gt}^i})^2 & |\mbf{D}^i - \mbf{D_{gt}^i}| \leq \delta \\ \delta (|\mbf{D}^i - \mbf{D_{gt}^i}| - \frac{1}{2} \delta) & \text{otherwise} \end{cases}   
    \end{align}
    \item Scale invarient loss :
        \begin{align}
            \text{Scale inv} = \frac{1}{2N} \sum_{i=0}^{N} \Big( \log(\mbf{D}^i) - \log(\mbf{D_{gt}^i}) + \frac{1}{N} \sum_{i=0}^{N} \big( \log(\mbf{D}^i) - \log(\mbf{D_{gt}^i}) \big) \Big)
        \end{align}
\end{itemize}
\subsection{Monocular methods}
Eigen~\cite{Eigen2014}~\ea were among the first to investigate using deep learning for depth inference and developed a CNN network with two deep stacks. \reffig{eigen-arxh} shows the architecture. The first stack was used for preparing the input image and refining the depth map, the second stack was responsible for arranging the obtained coarse depth predictions with the objects in the scene.
\begin{figure}
    \centering
    \includegraphics[width=0.75\textwidth]{ch2/arch_vertical.pdf}
    \caption{Architecture for Eigen~\ea~\cite{Eigen2014}. Using a single image as input, the depth is reconstructed. The first stack was used for preparing the input image and refining the depth map, the second stack was responsible for arranging the obtained coarse depth predictions with the objects in the scene. Adopted from~\cite{Eigen2014}}
    \label{fig:eigen-arxh}
\end{figure}
This approach has led to an increased focus on convolutional architectures for depth prediction, with methods such as CLIFFNet~\cite{Wang2020} and Transformer-based networks like TransDepth~\cite{Zhao2021} and DPT~\cite{Ranftl2021}. These methods propose to replace convolution operations with Transformer layers, which further improve model performance. However, these methods have faced challenges with slow convergence and suboptimal solutions. Another approach to depth prediction involves discretizing continuous depth and treating it as a per-pixel classification problem. Methods like DORN~\cite{Fu2018}, which uses an ordinal classification depth estimation loss and an ASPP module~\cite{chen2017deeplab} to extract multi-level information, and Adabins\cite{Bhat2021}, which uses an adaptive bin's strategy to further improve the model performance. BinsFormer~\cite{Li2022} proposes classification-regression-based monocular depth estimation that utilizes Transformer layers for adaptive bin generation and a multiscale refinement strategy. 

\subsection{Stereo methods}
The field of stereo matching has undergone significant advancements in recent years, owing to the incorporation of deep learning techniques. Early works in this domain primarily focused on the use of Siamese networks for extracting patch-wise features or predicting matching costs~\cite{Luo2016,Zagoruyko2015,Zbontar2015}. Using end-to-end networks, researchers have been able to achieve more accurate results by jointly learning all steps of the stereo matching process~\cite{Shaked2017,Song2021}. Another line of research is the use of cost volume layer~\cite{Kendall2017}, which enables the network to perform per-pixel feature matching.
To improve the computational efficiency of stereo matching, researchers have proposed cascaded models~\cite{Pang2017,Yang2019,gidaris2017detect} that perform the search in disparity space in a coarse-to-fine fashion. In particular, the method proposed in~\cite{Pang2017} utilizes multiple residual blocks to improve the current disparity estimate. A more recent work~\cite{yang2019hierarchical} relies on a hierarchical cost volume, which allows the method to be trained on high-resolution images and generate different resolutions on demand.~\cite{tankovich2021hitnet} is inspired by classical stereo matching methods, it proposes an end-to-end learning approach that overcomes the issues of hand-crafted algorithms, while maintaining computational efficiency as it does not explicitly build a volume, and instead it relies on a fast multi-resolution initialization step, differentiable 2D geometric propagation and warping mechanisms to infer disparity hypotheses.
\subsection{Multi-view stereo (MVS)}
Multi-view stereo (MVS) addresses dense 3D representation using a series of calibrated images with known poses. Typically, a MVS network extracts image features by a CNN and constructs cost volume via plane sweep algorithm in which source images are warped to the reference view.~\cite{Yao2018} proposed MVSNet, which utilizes a 2D CNN to extract features and a 3D CNN for cost regularization in order to infer depth maps for large-scale MVS reconstruction. To address the high memory consumption of the 3D CNN, the cost volume is regularized with gated recurrent units (GRUs) in~\cite{Yao2019}. Additionally, Wei \ea~\cite{Wei2021}. proposed AA-RMVSNet, which employs adaptive aggregation and long short-term memory (LSTM) to further improve the performance of MVS reconstruction. Fast-MVSNet~\cite{yu2020fast}, was the first to propose a sparse cost volume to infer an initial sparse depth map and then optimizes the sparse depth map gradually.~\cite{Gu2020} constructed a cascade cost volume in a coarse-to-fine manner to recover a high-resolution depth map. \cite{Cheng2020} built adaptive thin volumes in multiple stages to progressively increase depth resolution and precision. Furthermore,~\cite{Yang2022} designed CVP-MVSNet, which utilizes a pyramid structure to iteratively refine depth maps.~\cite{Wang2021} introduced the traditional patchmatch stereo algorithm into a learning-based coarse-to-fine framework. While these learning-based methods have achieved significant success, they still face challenges such as match ambiguities and mismatches in challenging regions, likely due to insufficient global context and 3D-inconsistent representations.











\subsection{The generalization of supervised approaches}
As supervised methods rely on labeled datasets, the generalization of these models could be limited. Most of the benchmarks are predominately daytime and do not include complex situations such as weather variations. We have explored the possibility of using GANs in order to improve the generalization of the supervised method. Several works were proposed in the literature to improve the generalization using GANs, this includes applications such as domain adaptation~\cite{Kim2019,Sankaranarayanan2018,Yang2020,Vu2019}. \cite{porav2019don} leverage CycleGAN~\cite{zhu2017unpaired} to create a multi-domain labeled dataset. By translating a labeled daytime dataset into nighttime style. These images will be used to perform domain adaptation. Similarly, we have proposed to train an end-to-end model that performs at the same time style-transfer and domain adaptation~\cite{boulahbal:hal-03365983}. However, A fundamental problem with generative models is \textbf{hallucination}. These models tend to create outputs that are not consistent with the conditioning input variable. This could be problematic in domain adaptation. We have investigated this problem further, and we have discovered that the classical conditional GAN approach applied to these models is not fully conditional, and the discriminator does not learn this property of the data (\ie the conditionality). More information about the problem, the formulation, the validation protocol, and the results are presented in Appendix~\ref{ch:apdx}. In the following, we present the method and results of the \textit{acontario cGAN} on a depth prediction problem.   

\subsubsection{Classic cGAN}
\label{sec:ccgan}

Classical cGAN training is based on conditionally paired sets of data $\mathcal{C}(\mbf{x},\mbf{y})$ where $\mbf{x}\sim p(\mbf{x})$ is the condition variable and $\mbf{y}\sim p(\mbf{y}|\mbf{x})$ is the real training variable. The generator of a cGAN outputs a transformed set of data $\mathcal{C}_G(\mbf{x},\mbf{y}_G)$ composed of the generator output variable $\mbf{y}_G\sim p_G(\mbf{y})$ and the condition variable. These sets of data will be called "real-conditional" and "generated-conditional" respectively. 
The discriminator is defined as:
\begin{align}
    D(\mbf{x},\mbf{y}):=\mathcal{A}(f(\mbf{x},\mbf{y}))
    \label{eq:discriminator}
\end{align}
Where $f(.)$ is a neural network function of $\mbf{x}$ and $\mbf{y}$, and $\mathcal{A}$ is the activation function whose choice depends on the objective function. The classical cGAN objective function is defined as: 
\begin{align}
         \mathcal{L}_{adv}= \min_{G} \max_{D} \left(\: \mathbb{E}_{\mbf{x}\sim p(\mbf{x}),\mbf{y}\sim p(\mbf{y}|\mbf{x})}\big[log(D(\mbf{x},\mbf{y})]\big] +   \mathbb{E}_{\mbf{x}\sim p(\mbf{x})}\big[log[1 - D(\mbf{x},G(\mbf{x}))]\big] \right)
\label{eq:classic_loss}
\end{align}
The min-max activation function is defined as a Sigmoid $\mathcal{A}(\mbf{x})=\left({\frac{1}{1+e^{-\mbf{x}}}}\right)$.




\subsubsection{Acontrario conditionality loss}
\label{sec:consistency}




The proposed \ac cGAN approach~\cite{Boulahbal2021BMVC} is based on training with unconditionally paired sets of data, obtained by randomly shuffling or paring the original conditional sets of data. The \ac set is defined as $\mathcal{C}_U(\mbf{\tilde x},\mbf{y})$, where $\mbf{\tilde x}\sim p(\mbf{x})$ is the \ac conditional variable ($\mbf{\tilde x} \neq \mbf{x}$) and $\mbf{y}$ is the real training variable as in Section~\ref{sec:ccgan}. In this case $\mbf{\tilde x}$ and $\mbf{y}$ are independent. The generator of the \ac cGAN outputs a transformed set of data $\mathcal{C}_{UG}(\mbf{\tilde x},\mbf{y})$ composed of the generator output variable $\mbf{y}_G\sim p_G(\mbf{y})$ and the random variable $\mbf{\tilde x}$. These two sets of data will be called "real-\ac" and "generated-\act" respectively. The motivation to create these new sets is to train the discriminator to correctly classify unconditional data as false. Figure~\ref{fig:pipeline} shows the four possible pairings. In practice, random sampling of \ac pairs is carried out without replacement and attention is paid to not include any conditional variables into a same batch while processing.

In order to enforce conditionality between $\mbf{y}$ and $\mbf{x}$ an \ac term is proposed as:
\begin{align}
        \mathcal{L}_{ac}= \max_{D} \: & \left(\mathbb{E}_{\mbf{\tilde x} \sim p(\mbf{\tilde x}) ,\mbf{y}\sim p(\mbf{y})}\big[log(1 - D(\mbf{\tilde x},\mbf{y}))\big]  + 
        \mathbb{E}_{\mbf{\tilde x} \sim p(\mbf{\tilde x}) ,\mbf{x} \sim p(\mbf{x})}\big[log(1 - D(\mbf{\tilde x},G(\mbf{x})))\big] \right)
\label{eq:ac_loss}
\end{align}
The first term enforces the real-\act pairs to be classified as false. The second term enforces the generated-\act as false. The final loss is:
\begin{align}
    \mathcal{L}_{adv}^{'}  = \mathcal{L}_{adv}+ \mathcal{L}_{ac}
\label{eq:overall_loss}
\end{align}

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{ch3/im-to-depth.pdf}
    \caption{Qualitative results for depth prediction. The \ac cGAN shows better performance and more consistent prediction with respect to the input. The first row shows a case of mode collapse for the baseline as it ignores completely the input.}
    \label{fig:depth_qualitative}
\end{figure*}






\subsubsection{Experiement results}


The model is trained on the NYU Depth V2 Dataset~\cite{Silberman:ECCV12} to predict depth from monocular 2D-RGB images only. The official train/validation split of $795$ pairs is used for training and $694$ pairs are used for validation. The dataset images are resized to have a resolution of $256\times256$. The experiment is repeated 6 times, and the mean and standard deviation are reported.


Table~\ref{tab:Depth_stat} shows the comparison of the two models across different metrics. Clearly, the \ac cGAN reaches a better performance with log RMSE $0.3036$ versus $0.3520$ for the baseline (the mean is reported here). The qualitative results are shown in Figure~\ref{fig:depth_qualitative}.

\begin{table}   
    \centering
    \begin{tabular}{|c||c|c|c|c|}
         \hline
         Method &  RMSE $\log$ & si$\log$ & $\log_{10}$ & abs rel \\
         \hline
         baseline & 0.3520$\pm$ 0.0016 & 28.54$\pm$ 0.1932  & 0.1247 $\pm$ 0.0005 & 0.3318$\pm$ 0.0026 \\
         \hline
         \ac & \textbf{0.3036}$\pm$ 0.0055  & \textbf{23.51}$\pm$ 0.1932 & \textbf{0.1079} $\pm$ 0.0021 & \textbf{0.2868} $\pm$ 0.0093\\
         \hline
    \end{tabular}
    \vspace{0.2cm}
    \caption{\small	 Monocular Depth prediction experiments were repeated on the baseline and \ac cGANs 6 times with different seeds. The mean and standard deviation are reported for each metric. The results shows that the \ac cGAN outperforms the baseline on the depth metric~\cite{eigen2014depth}.
    }
    \label{tab:Depth_stat}
    
\end{table}



For the classical cGAN, the discriminator is optimized only to distinguish real and generated samples, its decision boundary is independent of the conditional variable. The baseline cGAN architecture will not penalize the generation of outputs belonging to the target domain, but that do not correspond to the input (\ie not conditional pair). Not only does this leave the generator with a larger search space (the generator is less efficient), but it can allow mode collapse, whereby the generator always produces the same output. The \ac loss explicitly avoids this by penalizing unconditional generation. As observed in the qualitative results, both methods generate smooth and depth that resemble the distribution of an indoor depth. However, for the cGAN the depth output is not consistent to the conditioning input. The model hallucinate a room, it has the ability to freely invent an output that has the distribution of the room depth map. The acontario method enforces the conditionality explicitly, and it is able to generate an accurate and a consistent input-output.  





























\subsection{Stereo methods}
These models leverage a binocular video in order to supervise the network. These models have several advantageous over monocular methods: the pose transformation between left and right camera pair is constant. This pose could be estimated using camera calibration before acquiring the data. The pair captures the scene simultaneously (with infinitesimal time delay), this makes the observation of the scene from the stereo pair static. furthermore, the problem of occlusion is handled better as there is more spatial and temporal context to be used to handle occlusion. Several methods were proposed in the literature\cite{Wang2022,Peng2021,Bello2021,Zhu2020,Watson2019,Pilzer2019,Godard2017,Garg2016}.~\cite{Garg2016} was the first to propose a differentiable warping that warps the left image into the right and vice versa.~\cite{Godard2017} proposes single image depth estimation using binocular stereo input. This paper proposes a novel training objective function that enforces consistency between the disparities produced relative to both left and right images.~\cite{Pilzer2019} proposes a distillation method using teacher/student networks. This method computes the inconsistencies between input and cycle-reconstructed images and exploits them to generate state-of-the-art depth predictions through a refinement network.~\cite{Watson2019} addresses the local minima problem of photometric loss in self-supervision by incorporating depth suggestions from off-the-shelf stereo algorithms.~\cite{Wang2022} proposes a novel depth representation called PlaneDepth, which uses orthogonal planes, to estimate depth distribution using a Laplacian Mixture Model. The approach addresses the problem of discontinuity caused by near frontal-parallel planes and boosts the robustness of the representation for occlusions. 

\subsection{MVS methods}
The first unsupervised MVS framework that utilizes end-to-end learning is proposed by UnsupMVS~\cite{khot2019learning}. In this framework, the source view images are reversely warped to the reference view using a predicted depth map. JDACS~\cite{xu2021self} enforces cross-view consistency of extracted semantic features and utilizes non-negative matrix factorization to supervise the segmentation map. However, this approach still requires a pre-trained semantic feature extraction backbone and suffers from unstable convergence of cross-view semantic consistency, leading to unreliable supervision. U-MVSNet~\cite{xu2021digging} improves the supervision by employing a flow-depth consistency loss to generate pseudo labels for uncertainty-aware consistency, but it cannot be trained end-to-end and requires complex pre-training and fine-tuning. Self-supervised CVP-MVSNet~\cite{yang2021self} learns depth pseudo labels with unsupervised pre-training, followed by iterative self-supervised training to refine the pseudo label. However, it is still affected by ambiguous supervision. Moreover, these unsupervised and self-supervised methods lack an occlusion-aware module, leading to incomplete reconstruction of point clouds from different viewing directions. RC-MVSNet~\cite{chang2022rc} uses neural rendering to alleviate occlusions and non-Lambertian surfaces. It includes a depth rendering consistency loss to constrain geometry features close to the object surface and a reference view synthesis loss to provide consistent supervision.


\subsection{Discussion of self-supervised versus supervised monocular depth prediction approaches}



~\reftab{ssl-vs-sup} shows the comparison between self-supervised and supervised depth prediction methods on the KITTI benchmark~\cite{Geiger2012CVPR}, the supervised approaches represent the state-of-the-art in depth prediction tasks, yielding higher accuracy compared to SSL methods. Despite this observation, it is important to note that this comparison may not fully reflect the potential of SSL methods in depth prediction.

Self-Supervised Learning (SSL) methods offer a compelling advantage in training depth prediction models on large-scale datasets without the need for depth annotations. Unlike supervised methods, which heavily rely on annotated labels, SSL methods can leverage abundant unlabeled data to achieve high accuracy and overcome scalability limitations. By designing effective pretext tasks, such as image warping, SSL methods capture the structure and semantics of the data. The quality of self-supervised representations has been observed to improve logarithmically~\cite{goyal2019scaling} with the volume of unlabeled pretraining data, highlighting the vast potential of SSL methods in depth prediction tasks. This means that eventually, if SSL methods were trained on enough large scale datasets, these methods will surpass the supervised method. Furthermore, advancements in pretext tasks and model architectures for SSL can lead to even more accurate and robust depth predictions.

Therefore, it is important to consider the limitations of comparing self-supervised methods and supervised methods solely on a single dataset, such as KITTI. Such comparisons might not fully explore the capabilities of SSL methods, as they are confined to training on a specific dataset.





\begin{table*}
\centering
\footnotesize
\begin{tabular}{|c|l ||c c c c ||c c c|}
\hline
Approach & Method & Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline
Supervised 
 & Eigen~\cite{Eigen2014} & 0.203 & 1.548 & 0.282 & 6.307 & 0.702 & 0.898 & 0.967 \\
 & Kuznietsov et al~\cite{kuznietsov2017semi} & 0.113 & 0.741 & 4.621 & 0.189 & 0.862 & 0.960 & 0.986 \\
  & DORN~\cite{Fu2018} & 0.072  & 0.307 & 2.727 & 0.120 & 0.932 & 0.984 & 0.994 \\
 & TransDepth~\cite{Zhao2021} & 0.064 & 0.252 & 2.755 &  0.098 & 0.956 & 0.994 & 0.999 \\
 & DPT~\cite{Ranftl2021}  & 0.062 & –& 2.573 & 0.092 & 0.959 & 0.995 & 0.999 \\
 &Adabins~\cite{Bhat2021} & 0.058 & 0.190 & 2.360 & 0.088 & 0.964 & 0.995 &  0.999 \\
&BinsFormer~\cite{Li2022} &0.052 & 0.151 & 2.098 & 0.079 & 0.974 & 0.997 & 0.999 \\

       
\hline  
Self-supervised &
SfMlearner~\cite{Zhou2017}  & 0.183 & 1.595 & 6.709 & 0.270 & 0.734& 0.902 &0.959 \\
&Monodepth2~\cite{Godard2019}  & 0.115 & 0.903 & 4.863 & 0.193 & 0.877 & 0.959 & 0.981\\
&Lee \ea~\cite{lee2021attentive}  &  0.113 & 0.835 & 4.693 & 0.191 & 0.879 & 0.961 & 0.981 \\
&SGDepth~\cite{Klingner2020}  & 0.113 & 0.835 & 4.693 & 0.191 & 0.879 & 0.961 & 0.981\\
&SAFENet~\cite{lou2020safenet}& 0.112 & 0.788 & 4.582 & 0.187 & 0.878 & 0.963 & 0.983 \\
&Insta-DM~\cite{lee2021learning}& 0.112& 0.777 &4.772 &0.191& 0.872& 0.959& 0.982 \\
&PackNetSfm~\cite{Rares2020} & 0.111 & 0.785 & 4.601 & 0.189 & 0.878 & 0.960 & 0.982\\
&MonoDepthSeg~\cite{safadoust2021self} & 0.110 & 0.792 & 4.700 & 0.189 & 0.881 & 0.960 & 0.982 \\
&Johnston \ea~\cite{johnston2020self}  & 0.106 & 0.861 & 4.699 & 0.185 & \underline{0.889} & 0.962 & 0.982 \\
&Manydepth~\cite{Watson2021}  & 0.098 & 0.770 & 4.459 & 0.176 & 0.900 & 0.965 & 0.983 \\
\hline
\end{tabular}
\caption{Quantitative performance comparison of on the KITTI benchmark with Eigen split~\cite{Geiger2012CVPR}. For Abs Rel, Sq Rel, RMSE and RMSE log lower is better, and for $\delta < 1.25$, $\delta < 1.25^2$ and $\delta < 1.25^3$ higher is better.}
\label{tab:ssl-vs-sup}
\end{table*}





==> ch6/results_ablation.tex <==
 \begin{table*}
\centering
\footnotesize
\begin{tabular}{|l||c c c c ||c c c c| c c c |}
\hline 
experiment & Use vae & share prediction & Instance warping & stereo &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$&
\hline \hline


E1 &  & & & &                       
0.114  &   0.809  &   4.702  &   0.187  &   0.875  &   0.961  &   0.983     \\ 

E2 & \checkmark & & & &             
0.113  &   0.860  &   4.812  &   0.190  &   0.870  &   0.958  &   0.982    \\

E3 &  & \checkmark & & &           
0.110  &   0.805  &   4.678  &   0.187  &   0.879  &   0.961  &   0.983   \\



E4 & \checkmark  & \checkmark & & &     
0.112  &   0.844  &   4.754  &   0.189  &   0.876  &   0.960  &   0.981  \\

\hline \hline 

E5 &  & & \checkmark& &            
0.118  &   0.905  &   4.881  &   0.194  &   0.868  &   0.957  &   0.981  \\

E6 &  & & &\checkmark &             
0.110  &   0.765  &   4.809  &   0.192  &   0.876  &   0.957  &   0.981    \\

E7 & \checkmark &  & &\checkmark &             
0.110  &   0.770  &   4.884  &   0.193  &   0.877  &   0.957  &   0.980 \\

E8 & & \checkmark  & &  \checkmark  &             
 0.109  &   0.762  &   4.811  &   0.191  &   0.877  &   0.957  &   0.981   \\

\hline 

\end{tabular}
\caption{$t=0$ Quantitative performance comparison of on the KITTI benchmark.}
%\caption{Quantitative performance comparison of on the KITTI benchmark with Eigen split~\cite{Geiger2012CVPR}. For Abs Rel, Sq Rel, RMSE and RMSE log lower is better, and for $\delta < 1.25$, $\delta < 1.25^2$ and $\delta < 1.25^3$ higher is better. The Supervision column illustrates the traing modalities: (M) raw images (S)Semantic, (F) optical flow, (TS) Teacher-student. At test-time, all monocular methods (M) scale the estimated depths with median ground-truth LiDAR.The best scores are bold and the second are underlined}
\label{tab:results}
\end{table*}




 \begin{table*}
\centering
\footnotesize
\begin{tabular}{|l||c c c c ||c c c c| c c c|}
\hline 
experiment & Use vae & share prediction & Instance warping & stereo &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline \hline  
E1 &  & & & &                       
0.125  &   0.994  &   4.986  &   0.201  &   0.859  &   0.954  &   0.980   \\ 

E2 & \checkmark & & & &             
 0.124  &   1.038  &   5.128  &   0.205  &   0.855  &   0.950  &   0.978    \\

E3 &  & \checkmark & & &           
0.121  &   0.989  &   5.026  &   0.203  &   0.863  &   0.951  &   0.978   \\



E4 & \checkmark  & \checkmark & &  &            
  0.125  &   1.082  &   5.191  &   0.207  &   0.859  &   0.950  &   0.977     \\

\hline \hline 
E5 &  & & \checkmark& &            
0.129  &   1.124  &   5.244  &   0.209  &   0.851  &   0.948  &   0.976    \\

E6 &  & & &\checkmark &             
0.118  &   0.871  &   5.034  &   0.204  &   0.864  &   0.951  &   0.978     \\

E7 & \checkmark  & & &\checkmark &             
0.118  &   0.887  &   5.112  &   0.204  &   0.864  &   0.950  &   0.977  \\
E8 &  & \checkmark & &  \checkmark  &             
 0.116  &   0.848  &   4.951  &   0.200  &   0.868  &   0.953  &   0.978  \\

\hline \hline

\end{tabular}
\caption{$t=1$  Quantitative performance comparison of on the KITTI benchmark.}
%\caption{Quantitative performance comparison of on the KITTI benchmark with Eigen split~\cite{Geiger2012CVPR}. For Abs Rel, Sq Rel, RMSE and RMSE log lower is better, and for $\delta < 1.25$, $\delta < 1.25^2$ and $\delta < 1.25^3$ higher is better. The Supervision column illustrates the traing modalities: (M) raw images (S)Semantic, (F) optical flow, (TS) Teacher-student. At test-time, all monocular methods (M) scale the estimated depths with median ground-truth LiDAR.The best scores are bold and the second are underlined}
\label{tab:results}
\end{table*}



 \begin{table*}
\centering
\footnotesize
\begin{tabular}{|l||c c c c ||c c c c| c c c|}
\hline 
experiment & Use vae & share prediction & Instance warping & stereo &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline
E1 &  & & & &                       
 0.148  &   1.300  &   5.468  &   0.226  &   0.823  &   0.939  &   0.972     \\ 

E2 & \checkmark & & & &             
 0.146  &   1.317  &   5.553  &   0.227  &   0.823  &   0.935  &   0.971    \\

E3 &  & \checkmark & & &           
   0.146  &   1.295  &   5.493  &   0.227  &   0.824  &   0.935  &   0.971   \\



E4 & \checkmark  & \checkmark & &  &            
0.147  &   1.363  &   5.624  &   0.230  &   0.824  &   0.935  &   0.970   \\

\hline \hline 
E5 &  & & \checkmark& &            
 0.152  &   1.485  &   5.744  &   0.233  &   0.818  &   0.933  &   0.970    \\

E6 &  & & &\checkmark &             
0.137  &   1.106  &   5.407  &   0.223  &   0.833  &   0.938  &   0.972 \\

E7 &\checkmark  &  & &\checkmark &             
0.136  &   1.128  &   5.456  &   0.224  &   0.833  &   0.937  &   0.971 \\

E8 &  &\checkmark & &  \checkmark  &             
 0.137  &   1.106  &   5.342  &   0.221  &   0.834  &   0.939  &   0.972  \\

\hline 

\end{tabular}
\caption{$t=3$  Quantitative performance comparison of on the KITTI benchmark.}
%\caption{Quantitative performance comparison of on the KITTI benchmark with Eigen split~\cite{Geiger2012CVPR}. For Abs Rel, Sq Rel, RMSE and RMSE log lower is better, and for $\delta < 1.25$, $\delta < 1.25^2$ and $\delta < 1.25^3$ higher is better. The Supervision column illustrates the traing modalities: (M) raw images (S)Semantic, (F) optical flow, (TS) Teacher-student. At test-time, all monocular methods (M) scale the estimated depths with median ground-truth LiDAR.The best scores are bold and the second are underlined}
\label{tab:results}
\end{table*}






 \begin{table*}
\centering
\footnotesize
\begin{tabular}{|l||c c c c ||c c c c| c c c|}
\hline 
experiment & Use vae & share prediction & Instance warping & stereo &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline \hline

ForecastMonodepth2 & & & & &
0.201  &   1.588   &   0.275  &   6.166 &   0.702 &  0.897  &   0.960\\
ICPR paper & & & & &
0.178  &  1.645   &   0.257 &   6.196 &   0.761  &   0.914  &   0.964 \\
\hline \hline

E1 &  & & & &                       
0.167  &   1.545  &   5.851  &   0.243  &   0.793  &   0.926  &   0.967 \\ 

E2 & \checkmark & & & &             
0.166  &   1.563  &   5.909  &   0.244  &   0.790  &   0.923  &   0.966    \\

E3 &  & \checkmark & & &           
0.165  &   1.489  &   5.805  &   0.245  &   0.792  &   0.921  &   0.964   \\



E4 & \checkmark  & \checkmark & &  &            
0.168  &   1.624  &   5.968  &   0.248  &   0.791  &   0.922  &   0.965    \\

\hline \hline 

E5 &  & & \checkmark& &            
0.170  &   1.711  &   6.082  &   0.250  &   0.788  &   0.920  &   0.964    \\

E6 &  & & &\checkmark &             
 0.156  &   1.312  &   5.720  &   0.242  &   0.799  &   0.924  &   0.966    \\

E7 & \checkmark &  & &\checkmark &             
0.155  &   1.328  &   5.792  &   0.241  &   0.799  &   0.925  &   0.967 \\

E8 &  & \checkmark & &  \checkmark  &             
 0.153  &   1.323  &   5.730  &   0.239  &   0.803  &   0.926  &   0.967    \\

\hline 

\end{tabular}
\caption{$t=5$  Quantitative performance comparison of on the KITTI benchmark.}
%\caption{Quantitative performance comparison of on the KITTI benchmark with Eigen split~\cite{Geiger2012CVPR}. For Abs Rel, Sq Rel, RMSE and RMSE log lower is better, and for $\delta < 1.25$, $\delta < 1.25^2$ and $\delta < 1.25^3$ higher is better. The Supervision column illustrates the traing modalities: (M) raw images (S)Semantic, (F) optical flow, (TS) Teacher-student. At test-time, all monocular methods (M) scale the estimated depths with median ground-truth LiDAR.The best scores are bold and the second are underlined}
\label{tab:results}
\end{table*}

==> ch6/results_generalization.tex <==


\begin{table*}
\centering
\footnotesize
\begin{tabular}{|l |cc||c c c c ||c c c|}
\hline
Method & Known intrinsic & Resolution &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline \hline  
Manydepth~\cite{}& \checkmark
 & 640$\times$192  & 0.098 & 0.770 & 4.459 & 0.176 & 0.900& 0.965 & 0.983 \\\text
 Manydepth~\cite{}& 
 & 640$\times$192  &  0.112  &   0.839  &   4.626  &   0.187  &   0.881  &   0.962  &   0.983  \\
  \hline \hline
DepthFormer~\cite{}& \checkmark   & 640$\times$192  & 0.090 & 0.661 & 4.149 & 0.175  & 0.905 & 0.967  & 0.984 \\
DepthFormer~\cite{}&  & 640$\times$192  & 0.125   &  0.893   &  4.713   &  0.206 & 0.849   & 0.949 &  0.977 \\
 \hline \hline
Ours& & 640$\times$192 & 0.107  &   0.797  &   4.614  &   0.185  &   0.889  &   0.963  &   0.982  \\
\hline 

\end{tabular}
\caption{Quantitative performance comparison of on the KITTI benchmark.}
\label{tab:results}
\end{table*}




\begin{table*}
\centering
\footnotesize
\begin{tabular}{|l| c||c c c c |c c c|}
\hline  
Method& Known intrinsic  &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline  \hline  
Manydepth~\cite{}& \checkmark  & 0.169  &   1.787  &   8.352  &   0.236  &   0.749  &   0.932  &   0.978  \\
Manydepth~\cite{}&  & 0.165  &   1.749  &   8.304  &   0.232  &   0.761  &   0.933  &   0.978 \\

DepthFormer~\cite{} &\checkmark &   0.213  &   2.291  &   8.978  &   0.292  &   0.633  &   0.877  &   0.957  \\

DepthFormer~\cite{}&   &  0.177  &   2.022  &   8.840  &   0.257  &   0.727  &   0.902  &   0.963  \\
Ours&  & 0.153  &   1.792  &   8.890  &   0.235  &   0.771  &   0.920  &   0.974  \\
\hline 

\end{tabular}
\caption{Quantitative performance comparison of on the Cityscapes.}
\label{tab:results}
\end{table*}




\begin{table*}
\centering
\footnotesize
\begin{tabular}{|l||c c c c c c c c|}
\hline 
Conditions & Method  &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline \hline
\multirow{3}{*}{\textbf{Rain sequence}} 
& Manydepth~\cite{} & 0.325  &   3.622  &   8.300  &   0.342  &   0.519  &   0.781  &   0.919  \\
& DepthFormer~\cite{} & 0.438  &   5.596  &   9.618  &   0.437  &   0.468  &   0.698  &   0.838  \\
& Ours& 0.284  &   3.064  &   7.934  &   0.313  &   0.561  &   0.821  &   0.937  \\
\hline

%\multirow{3}{*}{\textbf{Night sequence}} 
%& Manydepth~\cite{} &   0.422  &   5.304  &  11.154  &   0.451  &   0.408  &   0.664  &   0.834  \\
%& DepthFormer~\cite{}& 0.562  &   7.935  &  11.245  &   0.548  &   0.388  &   0.636  &   0.783  \\
%& Ours&      0.348  &   4.294  &  10.832  &   0.395  &   0.455  &   0.708  &   0.881  \\
%\hline \hline
\multirow{3}{*}{\textbf{Snow sequence}} 
& Manydepth~\cite{} &   0.328  &   3.694  &   8.712  &   0.367  &   0.505  &   0.766  &   0.902  \\
& DepthFormer~\cite{}&   0.441  &   5.551  &   9.486  &   0.448  &   0.477  &   0.718  &   0.844  \\
& Ours&     0.276  &   2.818  &   8.183  &   0.328  &   0.544  &   0.813  &   0.935  \\
\hline \hline


\multirow{3}{*}{\textbf{Overcast sequence}} 
& Manydepth~\cite{} &   0.247  &   3.018  &   6.442  &   0.278  &   0.668  &   0.836  &   0.924  \\
& DepthFormer~\cite{}& 0.359  &   4.980  &   7.167  &   0.357  &   0.606  &   0.769  &   0.865  \\
& Ours&      0.238  &   2.979  &   6.725  &   0.278  &   0.670  &   0.832  &   0.926  \\
\hline 

\end{tabular}
\caption{Quantitative performance comparison of on the Robotcar dataset night sequence}
\label{tab:results}
\end{table*}

